Duet: An Expressive Higher-order Language and Linear Type System for Statically Enforcing Differential Privacy

During the past decade, differential privacy has become the gold standard for protecting the privacy of individuals. However, verifying that a particular program provides differential privacy often remains a manual task to be completed by an expert in the field. Language-based techniques have been proposed for fully automating proofs of differential privacy via type system design, however these results have lagged behind advances in differentially-private algorithms, leaving a noticeable gap in programs which can be automatically verified while also providing state-of-the-art bounds on privacy. We propose Duet, an expressive higher-order language, linear type system and tool for automatically verifying differential privacy of general-purpose higher-order programs. In addition to general purpose programming, Duet supports encoding machine learning algorithms such as stochastic gradient descent, as well as common auxiliary data analysis tasks such as clipping, normalization and hyperparameter tuning - each of which are particularly challenging to encode in a statically verified differential privacy framework. We present a core design of the Duet language and linear type system, and complete key proofs about privacy for well-typed programs. We then show how to extend Duet to support realistic machine learning applications and recent variants of differential privacy which result in improved accuracy for many practical differentially private algorithms. Finally, we implement several differentially private machine learning algorithms in Duet which have never before been automatically verified by a language-based tool, and we present experimental results which demonstrate the benefits of Duet's language design in terms of accuracy of trained machine learning models.

==> constraints.tex <==
\section{Solving Type-Level Constraints}
\todo{No idea what to put in here}


==> extra.tex <==

% \begin{comment}
% \subsection{Hyperparameter Tuning}
% 
% Each of the gradient descent algorithms we have seen so far require a setting for the {{\color{\colorMATH}\ensuremath{\eta }}} hyperparameter. When privacy is not a concern, hyperparameters like {{\color{\colorMATH}\ensuremath{\eta }}} are typically tuned by comparing the accuracy of models trained using different settings. If this approach is taken in a differentially private setting, we must be careful to ensure that each trained model contributes to the overall privacy cost, and that the comparison of model accuracies is done in a differentially private way.
% 
% We can encode a simple algorithm for differentially private hyperparameter tuning using the exponential mechanism:
% 
% \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}
% \begin{array}{l
% }
% \cr  {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}SGD_{p} = p\lambda \hspace*{0.33em}\epsilon : {\mathbb{R}}[\epsilon ], \delta : {\mathbb{R}}[\delta ], \eta : {\mathbb{R}}[\eta ]
% \cr  \hspace*{1.00em}\hspace*{1.00em} X: cmatrix[L2 | n, m], y: matrix[n, 1] \Rightarrow  {.}\hspace{-1pt}{.}\hspace{-1pt}{.}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}
% \cr  {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}correct = \lambda \hspace*{0.33em}\theta : matrix[1, n], X: cmatrix[L2 | n, m],
% \cr  \hspace*{1.00em}\hspace*{1.00em} y: matrix[n, 1] \Rightarrow 
% \cr  \hspace*{1.00em} ({{\color{\colorSYNTAX}\texttt{csum}}}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{map-rows}}}\hspace*{0.33em}(\lambda \hspace*{0.33em}X_{i}, y_{i} .\hspace*{0.33em} \theta  \times  X_{i} = y_{i})\hspace*{0.33em}({{\color{\colorSYNTAX}\texttt{zip}}}\hspace*{0.33em}X\hspace*{0.33em}y))\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}
% \cr  {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}\theta s = {{\color{\colorSYNTAX}\texttt{map}}}\hspace*{0.33em}(\lambda \hspace*{0.33em}\eta  .\hspace*{0.33em} SGD_{p}\hspace*{0.33em}\epsilon \hspace*{0.33em}\delta \hspace*{0.33em}\eta \hspace*{0.33em}X\hspace*{0.33em}y)\hspace*{0.33em}[0.01, 0.1, 1.0]\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}
% \cr  {{\color{\colorSYNTAX}\texttt{exponential}}}[1, \epsilon ]\hspace*{0.33em}\theta s\hspace*{0.33em}\{ X, y .\hspace*{0.33em} \theta  \Rightarrow  correct\hspace*{0.33em}\theta \hspace*{0.33em}X\hspace*{0.33em}y\} 
%   \end{array}
% \vspace*{-1em}\end{gather*}\endgroup 
% 
% This algorithm trains one model per value of {{\color{\colorMATH}\ensuremath{\eta }}} in a set provided by the programmer ({{\color{\colorMATH}\ensuremath{[0.01, 0.1, 1.0]}}}), then uses the exponential mechanism to the number of correct answers each model produces on the training data (using the {{\color{\colorMATH}\ensuremath{correct}}} function).
% 
% If each invocation of {{\color{\colorMATH}\ensuremath{SGD_{p}}}} is {{\color{\colorMATH}\ensuremath{(\epsilon , \delta )}}}-differentially private, we can derive a bound of {{\color{\colorMATH}\ensuremath{(5\epsilon , 5\delta )}}}-differential privacy via standard composition; \system can derive this bound automatically, but can also do better---using zCDP or R\'enyi differential privacy, \system derives a bound of \todo{put the bound here}.
% \end{comment}


\subsection{Optimized Local Hashing}

Our final case study examines the settingof \emph{local} differential privacy, in which each individual adds noise to his or her data \emph{before} submitting it to a centralized aggregator. This setting contrasts with the \emph{central} model of differential privacy, which we have targeted in the previous examples, in which a trusted aggregator collects (un-noised) sensitive data and adds noise to the \emph{result of processing} the data.
%
The local model eliminates the need for a trusted aggregator, and is the basis for Google's RAPPOR~\cite{erlingsson2014rappor} and Apple's differential privacy system~\cite{apple}.

\system applies equally well in this setting. As a representative example, we implement the \emph{Optimized Local Hashing} (OLH)~\cite{DBLP:conf/uss/WangBLJ17} algorithm, which generalizes the classic idea of randomized response~\cite{warner1965randomized}. The algorithm's input is a single element of a finite domain of size {{\color{\colorMATH}\ensuremath{d}}} (e.g. in RAPPOR, the URL of the user's homepage); its output is a (randomized) element of the same domain. Note that OLH does not require {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy or iteration, so it could also be implemented in \dfuzz.
%
Our \system implementation requires a prime number {{\color{\colorMATH}\ensuremath{p}}} larger than {{\color{\colorMATH}\ensuremath{d}}}, in addition to {{\color{\colorMATH}\ensuremath{d}}} and the sensitive index {{\color{\colorMATH}\ensuremath{x}}} of the selected element. It leverages the {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{rand-resp}}}}}} construct (typing rule given below).
%{{\color{\colorSYNTAX}\texttt{OLH}}} &{}\mathrel{:: }{}& {\mathbb{N}}[d]@{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\infty }}}\endgroup }, \hspace*{1.00em} {\mathbb{N}}[p]@{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\infty }}}\endgroup }, \hspace*{1.00em} {\mathbb{N}}@{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{(\epsilon , 0)}}}\endgroup } \hspace*{1.00em} \multimap ^{*} {\mathbb{N}}
\begingroup \smallerplz
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{array}{l
  }{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{OLH}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{d}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup } \triangleq }}}\endgroup }
  \cr  \hspace*{1.00em} {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{a}}}\endgroup } \leftarrow  {{\color{\colorSYNTAX}\texttt{rand-nat}}}{{\color{\colorMATH}\ensuremath{({\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{1}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{p}}}\endgroup })}}}\mathrel{;}}}}}}}}\endgroup }
  \cr  \hspace*{1.00em} {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{b}}}\endgroup } \leftarrow  {{\color{\colorSYNTAX}\texttt{rand-nat}}}{{\color{\colorMATH}\ensuremath{({\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{0}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{p}}}\endgroup })}}}\mathrel{;}}}}}}}}\endgroup }
  \cr  \hspace*{1.00em} {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{{\color{\colorSYNTAX}\texttt{rand-resp}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{d}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{1}}}\endgroup }}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\epsilon }}}\endgroup }]\hspace*{0.33em}\{  {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{(({\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{a}}}\endgroup }\mathrel{\mathord{\cdotp }}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{b}}}\endgroup })\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{mod}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{p}}}\endgroup })\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{mod}}}\hspace*{0.33em}({\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{d}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{1}}}\endgroup })}}}\endgroup } \} }}}}}}}\endgroup }
  \end{array}
\cr \footnotesize
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}\begingroup\color{\colorMATH}
  \inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Rand-Resp}}}
  ]{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}[{{\color{\colorMATH}\ensuremath{n}}}]}}}}}}}\endgroup }}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{2} \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{R}}^{+}[{{\color{\colorMATH}\ensuremath{\epsilon }}}]}}}}}}}\endgroup }}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{3} + \mathrlap{\hspace{-0.5pt}{}\rceil }\lfloor \Gamma _{4}\mathrlap{\hspace{-0.5pt}\rfloor }\lceil {}^{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{n}}}\endgroup }}_{\{ {.}\hspace{-1pt}{.}\hspace{-1pt}{.}{,}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{n}}}}\endgroup }\} } \vdash  e_{3} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}}}}}}}}\endgroup }}}}\endgroup }
     }{
     {}\rceil {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1} {+} \Gamma _{2}}}}\endgroup }\lceil {}^{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }{,}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }} {+} {}\rceil {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{3}}}}\endgroup }\lceil {}^{{{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}} {+} \mathrlap{\hspace{-0.5pt}{}\rceil }\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{4}}}}\endgroup }\mathrlap{\hspace{-0.5pt}\rfloor }\lceil {}_{\{ \!{.}\hspace{-1pt}{.}\hspace{-1pt}{.}{,}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{n}}}}\endgroup }\!\} }^{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\epsilon }}}\endgroup }{,}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }}}}}}
     \vdash  {{\color{\colorSYNTAX}\texttt{\ensuremath{{{\color{\colorSYNTAX}\texttt{rand-resp}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup }{,}{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{2}}}}\endgroup }]{<}\!{.}\hspace{-1pt}{.}\hspace{-1pt}{.}{,}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{n}}}}\endgroup }\!{>}\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{3}}}}\endgroup }\} }}}} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}}}}}}}}\endgroup }
  }
  \endgroup \endgroup 
\vspace*{-1em}\end{gather*}\endgroup  \endgroup
To improve utility, OLH encodes the input using a family of hash functions before invoking randomized response; the use of {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{mod}}}}}} bounds sensitivity.
%Our \system implementation uses the {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{rand-resp}}}}}} construct for randomization, and the hashing performed using {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{mod}}}}}} bounds the sensitivity of {{\color{\colorMATH}\ensuremath{v_{p}}}}.
For a complete analysis of OLH, see Blocki et al.~\cite{DBLP:conf/uss/WangBLJ17}; \system derives the same state-of-the-art privacy bounds as the manual privacy proof.

% \begin{comment}
% \subsection{K-Means Clustering}
% 
% \todo{Fill this out}
% 
% \begin{verbatim}
% def kmeans(C, T, X, k, \epsilon ):
%     X = clip(X, (-72, 42), (-70, 43))
%     clusters = np.zeros(len(X))
%     \epsilon _i = \epsilon  / T
%     
%     for i in range(T):
%         for i in range(len(X)): # Assign centers
%             clusters[i] = np.argmin(dist(X[i], C))
% 
%         for i in range(k): # Move the centers
%             points = [X[j] for j in range(len(X)) if clusters[j] == i]
%             noisy_count = laplace_mech(len(points), 1, \epsilon _i / 2)
%             noisy_sum = laplace_mech(np.sum(points), (2, 1), \epsilon _1 / 2)
%             C[i] = noisy_sum / noisy_count
%     return C
% \end{verbatim}
% 
% \end{comment}


==> figures_scaling.tex <==

\begin{figure}
\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\mathrel{\mathord{\cdotp }}}\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{rcl@{\hspace*{1.00em}}c@{\hspace*{1.00em}}l
  } 0s   &{}\triangleq {}& 0
  \cr  s0   &{}\triangleq {}& 0
  \cr  r_{1}r_{2} &{}\triangleq {}& r_{1}r_{2}
  \cr  \infty s   &{}\triangleq {}& \infty  &{}{{\color{\colorTEXT}\textit{where}}}{}& s \neq  0
  \cr  s\infty    &{}\triangleq {}& \infty  &{}{{\color{\colorTEXT}\textit{where}}}{}& s \neq  0
  \end{array}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{rcl@{\hspace*{1.00em}}c@{\hspace*{1.00em}}l
  } (s\otimes \Gamma )(x)  &{}\triangleq {}& (ss^{\prime},\tau ) &{}{{\color{\colorTEXT}\textit{where}}}{}& (s^{\prime},\tau ) = \Gamma (x)
  \end{array}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{rcl@{\hspace*{1.00em}}c@{\hspace*{1.00em}}l
  } \infty +s   &{}\triangleq {}& \infty 
  \cr  s+\infty    &{}\triangleq {}& \infty 
  \cr  r_{1}+r_{2} &{}\triangleq {}& r_{1}+r_{2}
  \end{array}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \rightharpoonup  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{rcl@{\hspace*{1.00em}}c@{\hspace*{1.00em}}l
  } (\Gamma _{1}+\Gamma _{2})(x) &{}\triangleq {}& (s_{1}\oplus s_{2},\tau ) &{}{{\color{\colorTEXT}\textit{where}}}{}& (s_{1},\tau ) = \Gamma _{1}(x)\hspace*{1.00em}{{\color{\colorTEXT}\textit{and}}}\hspace*{1.00em}(s_{2},\tau ) = \Gamma _{2}(x)
  \end{array}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}^{\dagger } \in  ({{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}})\uplus ({{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}}) \endgroup}\endgroup \end{tabularx}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}0^{\dagger } \triangleq  0
    \hfill\hspace{0pt}r^{\dagger } \triangleq  1 \mathrel{{{\color{\colorTEXT}\textit{where}}}} r \neq  0
    \hfill\hspace{0pt}\infty ^{\dagger } \triangleq  \infty 
    \hfill\hspace{0pt}\Gamma ^{\dagger }(x) = \Gamma (x)^{\dagger }
    \hfill\hspace{0pt}
  \end{tabularx}
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\underline{\hspace{0.66em}\vspace*{5ex}}^{\dagger }}}}\endgroup }\rfloor  \in  ({\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{sens}}}}}}}\endgroup } \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}})\uplus ({\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}}}}}\endgroup } \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}}) \endgroup}\endgroup \end{tabularx}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{0^{\dagger }}}}\endgroup }\rfloor  \triangleq  0
    \hfill\hspace{0pt}\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r^{\dagger }}}}\endgroup }\rfloor  \triangleq  (1,1) \mathrel{{{\color{\colorTEXT}\textit{where}}}} r \neq  0
    \hfill\hspace{0pt}\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty ^{\dagger }}}}\endgroup }\rfloor  \triangleq  \infty 
    \hfill\hspace{0pt}\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma ^{\dagger }}}}\endgroup }\rfloor (x) = \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma ({\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{x}}}\endgroup })^{\dagger }}}}\endgroup }\rfloor 
    \hfill\hspace{0pt}
  \end{tabularx}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  (\epsilon _{1},\delta _{1})(\epsilon _{2},\delta _{2}) \triangleq  (\epsilon _{1}\epsilon _{2},\delta _{1}\delta _{2})
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  (\epsilon _{1},\delta _{1})+(\epsilon _{2},\delta _{2}) \triangleq  (\epsilon _{1}+\epsilon _{2},\delta _{1}+\delta _{2})
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}^{\dagger } \in  ({{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}})\uplus ({{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}}) \endgroup}\endgroup \end{tabularx}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}(0,0)^{\dagger } \triangleq  (0,0)
    \hfill\hspace{0pt}(\epsilon ,\delta )^{\dagger } \triangleq  (1,1) \mathrel{{{\color{\colorTEXT}\textit{where}}}} 0 \notin  \{ \epsilon ,\delta \} 
    \hfill\hspace{0pt}\infty ^{\dagger }     \triangleq  \infty 
    \hfill\hspace{0pt}
  \end{tabularx}
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 
\caption{Arithmetic, Scaling and Metafunctions}
\end{figure}


==> figures_semantics.tex <==

\begin{figure}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}D \in  {{\color{\colorMATH}\ensuremath{\operatorname{dom}}}} \triangleq  (X \in  {{\color{\colorMATH}\ensuremath{\operatorname{Set}}}}) \times  (\underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  X \times  X \rightarrow  {\mathbb{R}}\uplus \{ \infty \} )\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} {{\color{\colorMATH}\ensuremath{\operatorname{dom}}}} \endgroup}\endgroup \end{tabularx}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\| \langle X,\underline{\hspace{0.66em}\vspace*{5ex}}\rangle \|  = X\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \| \underline{\hspace{0.66em}\vspace*{5ex}}\|  \in  {{\color{\colorMATH}\ensuremath{\operatorname{dom}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{Set}}}} \endgroup}\endgroup \end{tabularx}
\vspace*{-1em}\end{gather*}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} [D@r,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},D@r] \rightrightarrows  D \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{l
  } [\langle X_{1},\underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }_{1}\underline{\hspace{0.66em}\vspace*{5ex}}\rangle @r_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\langle X_{n},\underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }_{n}\underline{\hspace{0.66em}\vspace*{5ex}}\rangle @r_{n}] \rightrightarrows  D \triangleq  f \in  X_{1} \times  {\mathord{\cdotp }}\hspace{-1pt}{\mathord{\cdotp }}\hspace{-1pt}{\mathord{\cdotp }} \times  X_{n} \rightarrow  X 
  \cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{where}}}\hspace*{1.00em} x_{i} \ominus _{i} x_{i}^{\prime} \leq  1 \implies   f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{i},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{i} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{i}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \leq  r
  \end{array}
\vspace*{-1em}\end{gather*}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} [D@p,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},D@p] \rightrightarrows ^{*} X \endgroup}\endgroup \end{tabularx}
\cr \begin{array}{l
  } [\langle X_{1},\underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }_{1}\underline{\hspace{0.66em}\vspace*{5ex}}\rangle @\langle \epsilon _{1},\delta _{1}\rangle ,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\langle X_{n},\underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }_{n}\underline{\hspace{0.66em}\vspace*{5ex}}\rangle @\langle \epsilon _{n},\delta _{n}\rangle ] \rightrightarrows ^{*} X \triangleq  f \in  X_{1} \times  {\mathord{\cdotp }}\hspace{-1pt}{\mathord{\cdotp }}\hspace{-1pt}{\mathord{\cdotp }} \times  X_{n} \rightarrow  {\mathcal{D}}(X)
  \cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{where}}}\hspace*{1.00em} x_{i} \ominus _{i} x_{i}^{\prime} \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{i},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{i}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n})] = x]} \leq  e^{\epsilon _{i}} + \delta _{i}
  \end{array}
\vspace*{-1em}\end{gather*}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{array}{c@{\hspace*{1.00em}}|@{\hspace*{1.00em}}c@{\hspace*{1.00em}}|@{\hspace*{1.00em}}rcl
  } {{\color{\colorMATH}\ensuremath{\operatorname{dom}}}}               & X \in  {{\color{\colorMATH}\ensuremath{\operatorname{Set}}}}             & \underline{\hspace{0.66em}\vspace*{5ex}}{\ominus }\underline{\hspace{0.66em}\vspace*{5ex}}     &{}\in {}& X \rightarrow  X \rightarrow  {\mathbb{R}}\uplus \{ \infty \} 
  \cr\hline  {{\color{\colorMATH}\ensuremath{\operatorname{nat}}}}               & {\mathbb{N}}                     & n_{1} \ominus  n_{2} &{}\triangleq {}& | n_{1} - n_{2} |
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{nat}}}}[n]            & \{ n\}                    & n_{1} \ominus  n_{2} &{}\triangleq {}& 0
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{real}}}}              & {\mathbb{R}}                     & r_{1} \ominus  r_{2} &{}\triangleq {}& | r_{1} - r_{2} |
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{real}}}}[r]           & \{ r\}                    & r_{1} \ominus  r_{2} &{}\triangleq {}& 0
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{data}}}}              & {\mathbb{R}}                     & r_{1} \ominus  r_{2} &{}\triangleq {}& \left\{ \begin{array}{l
                                                                 } 0\hspace*{0.33em}{{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em}r_{1}=r_{2}
                                                                 \cr  1\hspace*{0.33em}{{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em}r_{1}\neq r_{2}
                                                                 \end{array}\right.
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{matrix}}}}[n_{1},n_{2}](D^{\prime}) & X^{\prime n_{1}n_{2}}              & m_{1} \ominus  m_{2} &{}\triangleq {}& \sum \limits_{i,j}m_{1}[i,j] \ominus ^{\prime} m_{2}[i,j]
  \cr  D_{1}\boxplus D_{2}               & X_{1} \uplus  X_{2}               & x_{1} \ominus  x_{2} &{}\triangleq {}& \left\{ \begin{array}{l@{\hspace*{1.00em}}l
                                                                 } x_{1} \ominus _{1} x_{2}& {{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em} \{ x_{1},x_{2}\}  \subseteq  X_{1}
                                                                 \cr  x_{1} \ominus _{2} x_{2}& {{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em} \{ x_{1},x_{2}\}  \subseteq  X_{2}
                                                                 \cr  \infty        & {{\color{\colorTEXT}\textit{otherwise}}}
                                                                 \end{array}\right.
  \cr  D_{1}\boxtimes D_{2}               & X_{1} \times  X_{2}               & \langle x_{1 1},x_{1 2}\rangle  \ominus  \langle x_{2 1},x_{2 2}\rangle  &{}\triangleq {}& (x_{1 1} \ominus _{1} x_{2 1}) + (x_{1 2} \ominus _{2} x_{2 2})
  \cr  D_{1}\boxast D_{2}               & X_{1} \times  X_{2}               & \langle x_{1 1},x_{1 2}\rangle  \ominus  \langle x_{2 1},x_{2 2}\rangle  &{}\triangleq {}& (x_{1 1} \ominus _{1} x_{2 1}) \sqcup  (x_{1 2} \ominus _{2} x_{2 2})
  \cr  D_{1}\rightarrowtriangle _{s}D_{2}              & [X_{1}@s] \rightrightarrows  X_{2}           & f_{1} \ominus  f_{2}               &{}\triangleq {}& \bigsqcup \limits\{ f(x_{1}) \ominus _{2} f(x_{2}) \mathrel{|} x_{1} \ominus _{1} x_{2} \leq  1\} 
  \cr  {\mathcal{S}}_{r}(D^{\prime})              & ??                    & \tilde d_{1} \ominus  \tilde d_{2}           &{}\triangleq {}& ??
  \cr  [D_{1}@p_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},D_{n}@p_{n}]\rightarrowtriangle ^{*}D  & [D_{1}@X_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},D_{n}@p_{n}] \rightrightarrows ^{*} D  & f_{1} \ominus  f_{2}               &{}\triangleq {}& \left\{ \begin{array}{l
                                                                               } 0\hspace*{0.33em}{{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em}f_{1}=f_{2}
                                                                               \cr  1\hspace*{0.33em}{{\color{\colorTEXT}\textit{when}}}\hspace*{0.33em}f_{1}\neq f_{2}
                                                                               \end{array}\right.
  \end{array}               
\vspace*{-1em}\end{gather*}\endgroup                 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \underline{\hspace{0.66em}\vspace*{5ex}}\rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{type}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{dom}}}}\endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\begin{array}{rcl
  } \llbracket {{\color{\colorSYNTAX}\texttt{nat}}}\rrbracket               &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{nat}}}}
  \cr  \llbracket {{\color{\colorSYNTAX}\texttt{nat}}}[n]\rrbracket            &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{nat}}}}[n]
  \cr  \llbracket {{\color{\colorSYNTAX}\texttt{real}}}\rrbracket              &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{real}}}}
  \cr  \llbracket {{\color{\colorSYNTAX}\texttt{real}}}[r]\rrbracket           &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{real}}}}[r]
  \cr  \llbracket {{\color{\colorSYNTAX}\texttt{data}}}\rrbracket              &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{data}}}}
  \end{array}
\and\begin{array}{rcl
  } \llbracket {{\color{\colorSYNTAX}\texttt{matrix}}}[n_{1},n_{2}](\tau )\rrbracket  &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{matrix}}}}[n_{1},n_{2}](\llbracket \tau \rrbracket )
  \cr  \llbracket \tau _{1}+\tau _{2}\rrbracket               &{}\triangleq {}& \llbracket \tau _{1}\rrbracket  \boxplus  \llbracket \tau _{2}\rrbracket 
  \cr  \llbracket \tau _{1}\times \tau _{2}\rrbracket               &{}\triangleq {}& \llbracket \tau _{1}\rrbracket  \boxtimes  \llbracket \tau _{2}\rrbracket 
  \cr  \llbracket \tau _{1}\mathrel{\&}\tau _{2}\rrbracket               &{}\triangleq {}& \llbracket \tau _{1}\rrbracket  \boxast  \llbracket \tau _{2}\rrbracket 
  \cr  \llbracket \tau _{1}\multimap _{s}\tau _{2}\rrbracket              &{}\triangleq {}& \llbracket \tau _{1}\rrbracket  \rightarrowtriangle _{s} \llbracket \tau _{2}\rrbracket 
  \end{array}
\end{mathpar}\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \underline{\hspace{0.66em}\vspace*{5ex}}\vdash \underline{\hspace{0.66em}\vspace*{5ex}}\rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{type}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{Set}}}} \endgroup}\endgroup \end{tabularx}
\cr  \llbracket  \overbracketarg \Gamma {\{ x_{1} \mathrel{:}_{r_{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{r_{n}} \tau _{n}\} } \vdash  \tau  \rrbracket  \triangleq  \llbracket \tau _{1}\rrbracket  \mathrel{:}r_{1}, {.}\hspace{-1pt}{.}\hspace{-1pt}{.}, \llbracket \tau _{n}\rrbracket  \mathrel{:}r_{n} \rightrightarrows  \llbracket \tau \rrbracket 
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \underline{\hspace{0.66em}\vspace*{5ex}}\vdash \underline{\hspace{0.66em}\vspace*{5ex}}\rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{tcxt}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{type}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{Set}}}} \endgroup}\endgroup \end{tabularx}
\cr  \llbracket  \{ x_{1} \mathrel{:}_{\epsilon _{1},\delta _{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{\epsilon _{n},\delta _{n}} \tau _{n}\}  \vdash  \tau  \rrbracket  \triangleq  \llbracket \tau _{1}\rrbracket  \mathrel{:}\langle \epsilon _{1},\delta _{1}\rangle , {.}\hspace{-1pt}{.}\hspace{-1pt}{.}, \llbracket \tau _{n}\rrbracket  \mathrel{:}\langle \epsilon _{n},\delta _{n}\rangle  \rightrightarrows ^{*} \|  \llbracket \tau \rrbracket  \| 
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 
\caption{Semantics of Typing (1)}
\end{figure}




==> privacy_defs.tex <==
\section{Variants of Differential Privacy}
\label{sec:privacy_defns}



\begin{figure*}
  \footnotesize
\centering
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begin{array}{c@{\hspace*{1.00em}}rclrcl@{\hspace*{1.00em}}c@{\hspace*{1.00em}}c
     }  {{\color{\colorTEXT}\textit{\textbf{Variant}}}}               
      & \multicolumn{3}{c}{{{\color{\colorTEXT}\textbf{Privacy Cost}}}}                      
      & \multicolumn{3}{c}{{{\color{\colorTEXT}\textbf{Sequential Composition}}}}         
      & {{\color{\colorTEXT}\textbf{{{\color{\colorMATH}\ensuremath{k}}}-Loop}}} % Composition}}} 
      & {{\color{\colorTEXT}\textbf{Basic Mechanism}}}
     \cr  {{\color{\colorTEXT}\textit{RDP~\cite{mironov2017renyi}}}}     
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\alpha }}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\epsilon }}}\endgroup }}}}}}}}\endgroup }  &{}\mathrel{{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{|}}}}\endgroup }}{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup } 
      & (\alpha ,\epsilon _{1})+(\alpha ,\epsilon _{2})        &{}\triangleq {}&      (\alpha ,\epsilon _{1}+\epsilon _{2})           
      & (\alpha ,k\epsilon )                   
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{{\color{\colorSYNTAX}\texttt{gauss}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{s}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\alpha }}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\epsilon }}}\endgroup }]\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup }\} }}}}}}}\endgroup }
     \cr  {{\color{\colorTEXT}\textit{zCDP~\cite{bun2016concentrated}}}} 
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho }}}\endgroup }}}}}}}}\endgroup }  &{}\mathrel{{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{|}}}}\endgroup }}{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup } 
      & \rho _{1}+\rho _{2}          &{}\triangleq {}&       \rho _{1}+\rho _{2}               
      & k\rho                        
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{{\color{\colorSYNTAX}\texttt{gauss}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{s}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\rho }}}\endgroup }]\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup }\} }}}}}}}\endgroup }
     \cr  {{\color{\colorTEXT}\textit{tCDP~\cite{bun2018composable}}}}   
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho }}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\omega }}}\endgroup }}}}}}}}\endgroup }  &{}\mathrel{{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{|}}}}\endgroup }}{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup } 
      & (\rho _{1},\omega _{1})+(\rho _{2},\omega _{2})      &{}\triangleq {}&       (\rho _{1}+\rho _{2},\min(\omega _{1},\omega _{2})) 
      & (k\rho ,\omega )                   
      & {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{{\color{\colorSYNTAX}\texttt{sinh-normal}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{s}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\rho }}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\omega }}}\endgroup }]\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup }\} }}}}}}}\endgroup }
     \end{array}
    \hfill\hspace{0pt}
  \end{tabularx}
\vspace*{-1em}\end{gather*}\endgroup 
  \vspace{-1.5em}
  \caption{\system Extensions for Recent Variants of Differential Privacy}
  \vspace{-0.5em}
  \label{fig:typing_variants}
\end{figure*}



%% This bound on sensitivity is standard, but we have several choices in how to
%% approach the privacy proof. In fact, this definition satisfies a number of
%% \emph{different} bounds on privacy cost, based on the strategy used for the
%% other two parts of the analysis. Table~\ref{tbl:privacy_bounds_table}
%% summarizes the associated privacy bounds under the various possible strategies.

%% \begin{table} % {-{ tbl:privacy_bounds_table
%%   \begin{tabular}{l l}
%%     \hline
%%     \textbf{Approach}   & \textbf{Privacy Bound} \\
%%     \hline
%%     Std. comp.~\cite{privacybook} & {{\color{\colorMATH}\ensuremath{(k \epsilon , 0)}}}-DP\\
%%     Adv. comp.~\cite{privacybook} & {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta )}, \delta )}}}-DP\\
%%     Adv. comp.~\cite{BST}    & {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta ^{\prime})}, \delta  + k \delta ^{\prime})}}}-DP\\
%%     Mom. acct.~\cite{DPDL}          & {{\color{\colorMATH}\ensuremath{(4 \epsilon  \sqrt {k \log (1/\delta )}, \delta )}}}-DP\\
%%     RDP~\cite{mironov2017renyi}     & {{\color{\colorMATH}\ensuremath{(\alpha , k \epsilon )}}}-RDP\\
%%     zCDP~\cite{bun2016concentrated} & {{\color{\colorMATH}\ensuremath{k \rho }}}-zCDP\\
%%     tCDP~\cite{bun2018composable}   & {{\color{\colorMATH}\ensuremath{(k \rho , \omega )}}}-tCDP\\
%%     \hline
%%   \end{tabular}

%%   % \footnotesize
%%   % \begin{tabular}{l l l l}
%%   %   \textbf{Approach}   & \textbf{Clip} & \textbf{Noise}    & \textbf{Bound} \\
%%   %   \hline
%%   %   Std. comp.~\cite{privacybook} & {{\color{\colorMATH}\ensuremath{L1}}}     & Laplace  & {{\color{\colorMATH}\ensuremath{(k \epsilon , 0)}}}-DP\\
%%   %   Adv. comp.~\cite{privacybook} & {{\color{\colorMATH}\ensuremath{L1}}}     & Laplace  & {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta )}, \delta )}}}-DP\\
%%   %   Adv. comp.~\cite{BST}    & {{\color{\colorMATH}\ensuremath{L2}}}     & Gauss & {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta ^{\prime})}, \delta  + k \delta ^{\prime})}}}-DP\\
%%   %   Mom. acct.~\cite{DPDL}          & {{\color{\colorMATH}\ensuremath{L2}}}     & Gauss & {{\color{\colorMATH}\ensuremath{(4 \epsilon  \sqrt {k \log (1/\delta )}, \delta )}}}-DP\\
%%   %   RDP~\cite{mironov2017renyi}     & {{\color{\colorMATH}\ensuremath{L2}}}     & Gauss & {{\color{\colorMATH}\ensuremath{(\alpha , k \epsilon )}}}-RDP\\
%%   %   zCDP~\cite{bun2016concentrated} & {{\color{\colorMATH}\ensuremath{L2}}}     & Gauss & {{\color{\colorMATH}\ensuremath{k \rho }}}-zCDP\\
%%   %   tCDP~\cite{bun2018composable}   & {{\color{\colorMATH}\ensuremath{L2}}}     & Arsinh   & {{\color{\colorMATH}\ensuremath{(k \rho , \omega )}}}-tCDP\\
%%   % \end{tabular}

%%   \smallskip
%%   \caption{Statically Derivable Privacy Bounds for the \system Implementation of Gradient Descent in Figure~\ref{fig:gradient_descent}}
%%   \vspace{-0.5em}
%%   \label{tbl:privacy_bounds_table}
%% \end{table} % }-}

%% % \begin{itemize}[topsep=0.5mm,leftmargin=4mm]
%% % \itemsep1.0mm
%% % \item {{\color{\colorMATH}\ensuremath{k \epsilon }}}-differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L1}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Laplace noise scaled to {{\color{\colorMATH}\ensuremath{\epsilon }}}, under standard composition~\cite{SCS}.

%% % \item {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta )}, \delta )}}}-differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L1}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Laplace noise scaled to {{\color{\colorMATH}\ensuremath{\epsilon }}}, under advanced composition, for {{\color{\colorMATH}\ensuremath{\delta  > 0}}}~\cite{privacybook}.

%% % \item {{\color{\colorMATH}\ensuremath{(2 \epsilon  \sqrt {2 k \log (1/\delta ^{\prime})}, \delta  + k \delta ^{\prime})}}}-differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L2}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Gaussian noise with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{2 \log (1.25/\delta )}{\epsilon ^{2}}}}}, under advanced composition, for {{\color{\colorMATH}\ensuremath{\delta , \delta ^{\prime} > 0}}}~\cite{BST}.

%% % \item {{\color{\colorMATH}\ensuremath{(4 \epsilon  \sqrt {k \log (1/\delta )}, \delta )}}}-differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L2}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Gaussian noise with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{2 \log (1.25/\delta )}{\epsilon ^{2}}}}}, under the moments accountant, for {{\color{\colorMATH}\ensuremath{\delta  > 0}}}~\cite{DPDL}.

%% % \item {{\color{\colorMATH}\ensuremath{(\alpha , k \epsilon )}}}-R\'enyi differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L2}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Gaussian noise with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{\alpha }{2 \epsilon }}}}~\cite{mironov2017renyi}.

%% % \item {{\color{\colorMATH}\ensuremath{k \rho }}}-zero-concentrated differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L2}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds Gaussian noise with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{1}{2 \rho }}}}~\cite{bun2016concentrated}.

%% % \item {{\color{\colorMATH}\ensuremath{(k \rho , \omega )}}}-truncated concentrated differential privacy, when {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{clip-matrix}}}}}} clips the {{\color{\colorMATH}\ensuremath{L2}}} norm, and {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{noisy-grad}}}}}} adds \emph{arsinh} noise~\cite{bun2018composable}.

%% % \end{itemize}



%% % For iterative algorithms like gradient, the choice of mechanism and composition strategy can make a huge difference in the overall privacy cost of the algorithm. More recent definitions, like R\'enyi differential privacy and zero-concentrated differential privacy, generally produce much tighter bounds on privacy cost for iterative algorithms that use the Gaussian mechanism, since they are specifically designed for this purpose.

%% % \begin{figure}
%% %   \centering
%% %   \includegraphics[width=.4\textwidth]{privacy-cost.png}
%% %   \caption{Privacy Cost Comparison}
%% %   \label{fig:privacy_comparison}
%% % \end{figure}

\input{plot_privacy_bounds}


In addition to {{\color{\colorMATH}\ensuremath{\epsilon }}} and {{\color{\colorMATH}\ensuremath{(\epsilon , \delta )}}}-differential privacy, other variants of differential privacy with significant benefits have recently been developed. Three examples are R\'enyi differential privacy (RDP)~\cite{mironov2017renyi}, zero-concentrated differential privacy (zCDP)~\cite{bun2016concentrated}, and truncated concentrated differential privacy (tCDP)~\cite{bun2018composable}. Each one has different privacy parameters and a different form of sequential composition, summarized in Figure~\ref{fig:typing_variants}. The basic mechanism for RDP and zCDP is the Gaussian mechanism; tCDP uses a novel \emph{sinh-normal} mechanism~\cite{bun2018composable} which decays more quickly in its tails. All three can be converted to {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy, allowing them to be compared and composed with each other.
These three variants provide asymptotically tight bounds on privacy cost under composition, while at the same time eliminating the ``catastrophic'' privacy failure that can occur with probability {{\color{\colorMATH}\ensuremath{\delta }}} under {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy.

Due to their tight composition bounds, the use of these variants can yield dramatically more accurate algorithms for a given level of privacy. Figure~\ref{fig:privacy_comparison} plots the noise required to achieve {{\color{\colorMATH}\ensuremath{(1,10^{-5})}}}-differential privacy for an iterative algorithm (e.g. the gradient descent algorithm discussed in the next section), by the number of iterations performed. All three recent variants require the same noise level, and therefore their plots overlap. The noise level required for the recent variants is \emph{significantly} lower than that required for advanced composition or even the moments accountant; the lower level of noise results in greater accuracy for the \emph{same amount of privacy}.


%% %
%% In each of these variants, the ``{\sc Loop}'' rule for {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential
%% privacy is replaced by a simpler (yet still optimal) rule that merely iterates
%% the sequential composition privacy bounds.

%% Each of the bounds in Table~\ref{tbl:privacy_bounds_table} can be converted to {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy, allowing a direct comparison. For each one, Figure~\ref{fig:privacy_comparison} plots the variance of the per-iteration noise required to ensure {{\color{\colorMATH}\ensuremath{(1,10^{-5})}}}-differential privacy for the whole training process. The plot demonstrates that a good choice of composition theorem can produce the desired level of privacy using \emph{much less noise}, yielding a more accurate model.

The \system language and type system are designed for easy extension to new
    variants such as these. New variants can be supported by making three
    simple changes: (1) Modify the \emph{privacy cost} syntax {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }}}} to
    describe the privacy parameters of the new variant; (2) Modify the sum
    operator {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\underline{\hspace{0.66em}\vspace*{5ex}}{+}\underline{\hspace{0.66em}\vspace*{5ex}}}}}\endgroup } to reflect sequential composition in the new variant;
    and (3) Modify the typing for basic mechanisms (e.g. {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{gauss}}}}}}\endgroup }}}}) to
    reflect corresponding mechanisms in the new variant.

Figure~\ref{fig:typing_variants} summarizes the changes required for the three variants described here. The soundness proof also remains nearly identical: the only cases that require updating are the ones for \textsc{Return}, \textsc{Bind}, and the basic mechanisms. Importantly, the {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{p\lambda }}}}}}}\endgroup } and application cases do \emph{not} change, and neither does the sensitivity language.




\begin{comment}
\paragraph{R\'enyi Differential Privacy (RDP).}
%
R\'enyi differential privacy (RDP)~\cite{mironov2017renyi} is a relaxation of pure {{\color{\colorMATH}\ensuremath{\epsilon }}}-differential privacy that works by bounding R\'enyi divergence. RDP implies {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy, but not the reverse; RDP admits the Gaussian mechanism, but does not allow any mechanism that results in a ``catastrophic'' privacy failure with probability {{\color{\colorMATH}\ensuremath{\delta }}}.

The Gaussian mechanism with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \Delta ^{2} \alpha  / (2\epsilon )}}} provides {{\color{\colorMATH}\ensuremath{(\alpha , \epsilon )}}}-RDP for a value with sensitivity {{\color{\colorMATH}\ensuremath{\Delta }}}. For mechanisms {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{1}}}} and {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{2}}}} which provide {{\color{\colorMATH}\ensuremath{(\alpha , \epsilon _{1})}}} and {{\color{\colorMATH}\ensuremath{(\alpha , \epsilon _{2})}}}-RDP, respectively, their sequential composition provides {{\color{\colorMATH}\ensuremath{(\alpha , \epsilon _{1}+\epsilon _{2})}}}-RDP. This bound is tight for composition of the Gaussian mechanism \emph{automatically}---no separate advanced composition theorem is needed. RDP is closed under post-processing.

Figure~\ref{fig:typing_rdp} contains the changes to \system to support RDP. We modify the syntax of privacy costs to represent the {{\color{\colorMATH}\ensuremath{(\alpha ,\epsilon )}}} parameters, and define addition of privacy costs only for {{\color{\colorMATH}\ensuremath{\alpha }}}s that match. Typing will be successful for any choice of {{\color{\colorMATH}\ensuremath{\alpha }}}, as long as all uses of the Gaussian mechanism are consistent. We modify the proof in two cases: first, the \textsc{Gauss} case appeals to the proof of the Gaussian mechanism for RDP (\cite{mironov2017renyi}, Proposition 7); second, the \textsc{Bind} case appeals to the proof of sequential composition for RDP (\cite{mironov2017renyi}, Proposition 1).

% \begin{theorem}[Gaussian mechanism (RDP)~\cite{mironov2017renyi} (proposition 7)]
%   \label{thm:gauss_renyi}
  
%   \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
%   If {{\color{\colorMATH}\ensuremath{ | g(\gamma ) - g(\gamma [i\mapsto d]) | \leq  r }}}, then for {{\color{\colorMATH}\ensuremath{ f = \lambda  \gamma  .\hspace*{0.33em} g(\gamma ) + {\mathcal{N}}(0, \sigma ^{2}) }}} and {{\color{\colorMATH}\ensuremath{ \sigma ^{2} = \alpha  / (2\epsilon ) }}}, and all {{\color{\colorMATH}\ensuremath{\epsilon  > 0}}}:

%   \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d^{\prime}])) \leq  \epsilon 
%   \vspace*{-1em}\end{gather*}\endgroup 
%  \endgroup 
% \end{theorem}

% \begin{theorem}[Adaptive sequential composition (RDP)~\cite{mironov2017renyi} (proposition 1)]
%   \label{thm:let_renyi}

%   \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
%   \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} {{\color{\colorTEXT}\textit{If}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{1}(\gamma ) \|  f_{1}(\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime}
%   \cr  {{\color{\colorTEXT}\textit{and}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(d^{\prime \prime}, \gamma ) \|  f_{2}(d^{\prime \prime}, \gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime \prime}
%   \cr  {{\color{\colorTEXT}\textit{then}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(f_{1}(\gamma ),\gamma ) \|  f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}
%   \vspace*{-1em}\end{gather*}\endgroup 
%   \endgroup 
% \end{theorem}



\begin{figure}
  \footnotesize
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}
\cr \begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}\begingroup\color{\colorMATH}
  \begin{array}{rclcl@{\hspace*{1.00em}}l
  }  {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{p}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\in }}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{priv}}}}}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{\Coloneqq }}}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{\alpha }}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{\epsilon }}}}\endgroup }}}}} \mathrel{|} {{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup }                                                   & {{\color{\colorTEXT}\textit{privacy cost}}}
  \end{array}
  \endgroup \endgroup 
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
  % \cr  (\alpha ,\epsilon _{1})(\alpha ,\epsilon _{2}) \triangleq  (\alpha ,\epsilon _{1}\epsilon _{2})
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
  \cr  (\alpha ,\epsilon _{1})+(\alpha ,\epsilon _{2}) \triangleq  (\alpha ,\epsilon _{1}+\epsilon _{2})
\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
%\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}% \inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Bind}}}
  % ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }
  % \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup } \mathrel{:}_{\infty }{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }\} \uplus \Gamma _{2} \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  %    }{
  %    {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} + \Gamma _{2} \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup }\leftarrow e_{1}\mathrel{;}e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  % }
% \and\inferrule*[flushleft,lab={{\color{\colorTEXT}\textsc{\scriptsize Sample}}}
%   ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta  \vdash  \rho _{m^{\prime}} \mathrel{:} {{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}}}}}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\{ \rho _{m^{\prime}}\} }}}\endgroup }}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{2}\uplus \{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup }\mathrel{:}_{p_{1}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup }\mathrel{:}_{p_{2}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }\}  \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{m^{\prime}} \leq  \rho _{m}}}}\endgroup }
%      }{
%      {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\infty {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}}}}\endgroup }^{\dagger } 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{1}}]\hspace*{0.33em}\tau _{1}}}}\endgroup }\right\} 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{2}}]\hspace*{0.33em}\tau _{2}}}}\endgroup }\right\} 
%      +
%      \Gamma _{2} 
%   \\
%      \vdash  {{\color{\colorSYNTAX}\texttt{sample}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{on}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup } \Rightarrow  e_{2}\}  \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Gauss}}}
  ]{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[r]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\alpha ]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\epsilon ]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r\Gamma _{2}^{\dagger } \vdash  e_{4} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} }}}\endgroup }
     }{
     \infty \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}^{\dagger }}}}\endgroup }\rfloor  + (\alpha ,\epsilon )\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{2}^{\dagger }}}}\endgroup }\rfloor  \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{2}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{3}}}}\endgroup }]\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{4}}}}\endgroup }\}  \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}
  }
\end{mathpar}\endgroup 
\endgroup 

  \caption{Typing Rules for RDP}
  \label{fig:typing_rdp}
\end{figure}

\subsection{Zero-Concentrated Differential Privacy (zCDP)}

Like RDP, zero-concentrated differential privacy (zCDP)~\cite{bun2016concentrated} leverages R\'enyi divergence to provide tighter bounds on composition for the Gaussian mechanism, but it considers all {{\color{\colorMATH}\ensuremath{\alpha }}}s simultaneously and thus has only a single privacy parameter (called {{\color{\colorMATH}\ensuremath{\rho }}}). Like RDP, zCDP is a relaxation of {{\color{\colorMATH}\ensuremath{\epsilon }}}-differential privacy but stronger than {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy, it admits the Gaussian mechanism, and it is closed under post-processing.

The Gaussian mechanism with {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \Delta ^{2} / (2\rho )}}} provides {{\color{\colorMATH}\ensuremath{\rho }}}-zRDP for a value with sensitivity {{\color{\colorMATH}\ensuremath{\Delta }}}. For mechanisms {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{1}}}} and {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{2}}}} which provide {{\color{\colorMATH}\ensuremath{\rho _{1}}}} and {{\color{\colorMATH}\ensuremath{\rho _{2}}}}-zCDP, respectively, their sequential composition provides {{\color{\colorMATH}\ensuremath{\rho _{1}+\rho _{2}}}}-zCDP. As in RDP, tight composition is automatic.

Figure~\ref{fig:typing_zcdp} contains the changes to \system to support zCDP. We modify the proof in two cases: first, the \textsc{Gauss} case appeals to the proof of the Gaussian mechanism for zCDP (\cite{bun2016concentrated}, Proposition 1.6); second, the \textsc{Bind} case appeals to the proof of sequential composition for zCDP (\cite{bun2016concentrated}, Lemma 1.7).



\begin{figure}
  \footnotesize
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}
\cr \begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}\begingroup\color{\colorMATH}
  \begin{array}{rclcl@{\hspace*{1.00em}}l
  }  {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{p}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\in }}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{priv}}}}}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{\Coloneqq }}}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{\rho }}}}\endgroup }}}}} \mathrel{|} {{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup }                                                   & {{\color{\colorTEXT}\textit{privacy cost}}}
  \end{array}
  \endgroup \endgroup 
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
%  \cr  \rho _{1}\rho _{2} \triangleq  \rho _{1}\rho _{2}
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
  \cr  \rho _{1}+\rho _{2} \triangleq  \rho _{1}+\rho _{2}
\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
%\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}% \inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Bind}}}
  % ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }
  % \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup } \mathrel{:}_{\infty }{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }\} \uplus \Gamma _{2} \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  %    }{
  %    {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} + \Gamma _{2} \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup }\leftarrow e_{1}\mathrel{;}e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  % }
% \and\inferrule*[flushleft,lab={{\color{\colorTEXT}\textsc{\scriptsize Sample}}}
%   ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta  \vdash  \rho _{m^{\prime}} \mathrel{:} {{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}}}}}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\{ \rho _{m^{\prime}}\} }}}\endgroup }}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{2}\uplus \{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup }\mathrel{:}_{p_{1}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup }\mathrel{:}_{p_{2}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }\}  \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{m^{\prime}} \leq  \rho _{m}}}}\endgroup }
%      }{
%      {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\infty {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}}}}\endgroup }^{\dagger } 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{1}}]\hspace*{0.33em}\tau _{1}}}}\endgroup }\right\} 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{2}}]\hspace*{0.33em}\tau _{2}}}}\endgroup }\right\} 
%      +
%      \Gamma _{2} 
%   \\
%      \vdash  {{\color{\colorSYNTAX}\texttt{sample}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{on}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup } \Rightarrow  e_{2}\}  \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Gauss}}}
  ]{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[r]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\rho ]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r\Gamma _{2}^{\dagger } \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} }}}\endgroup }
     }{
     \infty \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}^{\dagger }}}}\endgroup }\rfloor  + \rho \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{2}^{\dagger }}}}\endgroup }\rfloor  \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{2}}}}\endgroup }]\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{3}}}}\endgroup }\}  \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}
  }
\end{mathpar}\endgroup 
\endgroup 

  \caption{Typing Rules for zCDP}
  \label{fig:typing_zcdp}
\end{figure}

\subsection{Truncated CDP (tCDP)}


Truncated concentrated differential privacy (tCDP)~\cite{bun2018composable} also bounds R\'enyi divergence, but relaxes the original definition of CDP to permit privacy amplification via subsampling. Despite this relaxation, tCDP is still stronger than {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy, and it is closed under post-processing.

The basic mechanism of tCDP is the \emph{sinh-normal} mechanism. For a sensitivity-{{\color{\colorMATH}\ensuremath{\Delta }}} value, adding noise drawn from
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} 8\Delta \omega \hspace*{0.33em} {{\color{\colorTEXT}\text{arsinh}}}(\frac{1}{8\Delta \omega } {\mathcal{N}}(0, \frac{\Delta ^{2}}{2\rho })) \vspace*{-1em}\end{gather*}\endgroup 
provides {{\color{\colorMATH}\ensuremath{(\rho , \omega )}}}-tCDP. For mechanisms {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{1}}}} and {{\color{\colorMATH}\ensuremath{{\mathcal{M}}_{2}}}} which provide {{\color{\colorMATH}\ensuremath{(\rho _{1}, \omega _{1})}}} and {{\color{\colorMATH}\ensuremath{(\rho _{2}, \omega _{2})}}}-tCDP, respectively, their sequential composition provides {{\color{\colorMATH}\ensuremath{\rho _{1}+\rho _{2}, \min(\omega _{1}, \omega _{2})}}}-tCDP. Tight composition is automatic.

Figure~\ref{fig:typing_zcdp} contains the changes to \system to support tCDP. In this case, we replace the \textsc{Gauss} rule (and its underlying basic mechanism) with a \textsc{Sinh-normal} rule for the new mechanism. We modify the proof in two cases: first, the \textsc{Sinh-normal} case appeals to the proof of the sinh-normal mechanism for tCDP (\cite{bun2018composable}, Theorem 17); second, the \textsc{Bind} case appeals to the proof of sequential composition for tCDP (\cite{bun2018composable}, Lemma 2).


\begin{figure}
  \footnotesize
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}
\cr \begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}\begingroup\color{\colorMATH}
  \begin{array}{rclcl@{\hspace*{1.00em}}l
  }  {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{p}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\in }}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{priv}}}}}}}\endgroup } &{}{\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{\mathrel{\Coloneqq }}}}\endgroup }{}& {\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{\rho }}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{\omega }}}}\endgroup }}}}} \mathrel{|} {{\color{\colorSYNTAX}\texttt{\ensuremath{\infty }}}}}}}\endgroup }                                                   & {{\color{\colorTEXT}\textit{privacy cost}}}
  \end{array}
  \endgroup \endgroup 
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
%  \cr  (\rho _{1},\omega _{1})(\rho _{1},\omega _{2}) \triangleq  (\rho _{1}\rho _{2},\omega _{1}\omega _{2})
%  \cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
  \cr  (\rho _{1},\omega _{1})+(\rho _{2},\omega _{2}) \triangleq  (\rho _{1}+\rho _{2},\min(\omega _{1},\omega _{2}))
\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
%\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}% \inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Bind}}}
  % ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }
  % \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup } \mathrel{:}_{\infty }{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup }\} \uplus \Gamma _{2} \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  %    }{
  %    {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} + \Gamma _{2} \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x}}}\endgroup }\leftarrow e_{1}\mathrel{;}e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }
  % }
% \and\inferrule*[flushleft,lab={{\color{\colorTEXT}\textsc{\scriptsize Sample}}}
%   ]{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta  \vdash  \rho _{m^{\prime}} \mathrel{:} {{\color{\colorSYNTAX}\texttt{\ensuremath{{\mathbb{N}}}}}}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{1} \vdash  e_{1} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\{ \rho _{m^{\prime}}\} }}}\endgroup }}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\Gamma _{2}\uplus \{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup }\mathrel{:}_{p_{1}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup }\mathrel{:}_{p_{2}}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{2}}}}\endgroup }\}  \vdash  e_{2} \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\rho _{m^{\prime}} \leq  \rho _{m}}}}\endgroup }
%      }{
%      {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\Delta }}}\endgroup },\infty {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}}}}\endgroup }^{\dagger } 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{1}}]\hspace*{0.33em}\tau _{1}}}}\endgroup }\right\} 
%      + 
%      \left\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup } \mathrel{:}_{{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\left(\tfrac{2\rho _{m^{\prime}}}{\rho _{m}},\tfrac{\rho _{m^{\prime}}}{\rho _{m}}\right)}}}\endgroup }p_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[\rho _{m},\rho _{n_{2}}]\hspace*{0.33em}\tau _{2}}}}\endgroup }\right\} 
%      +
%      \Gamma _{2} 
%   \\
%      \vdash  {{\color{\colorSYNTAX}\texttt{sample}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{on}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{2}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{3}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{x_{4}}}}\endgroup } \Rightarrow  e_{2}\}  \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHM}\renewcommand\colorSYNTAX{\colorSYNTAXM}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup }
%   }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Sinh-normal}}}
  ]{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[r]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\rho ]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\infty \Gamma _{1}^{\dagger } \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\omega ]}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r\Gamma _{2}^{\dagger } \vdash  e_{4} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} }}}\endgroup }
     }{
     \infty \lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{1}^{\dagger }}}}\endgroup }\rfloor  + (\rho ,\omega )\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{2}^{\dagger }}}}\endgroup }\rfloor  \vdash  {{\color{\colorSYNTAX}\texttt{sinh-normal}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{2}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{3}}}}\endgroup }]\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{4}}}}\endgroup }\}  \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}
  }
\end{mathpar}\endgroup 
\endgroup 

  \caption{Typing Rules for tCDP}
  \label{fig:typing_tcdp}
\end{figure}


\end{comment}


==> proofs.tex <==
\section{Theorems \& Lemmas}

\begin{theorem}[Gaussian mechanism]
  \label{thm:gauss}
  
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  If {{\color{\colorMATH}\ensuremath{ | g(\gamma ) - g(\gamma [i\mapsto d]) | \leq  r }}}, then for {{\color{\colorMATH}\ensuremath{ f = \lambda  \gamma  .\hspace*{0.33em} g(\gamma ) + {\mathcal{N}}(0, \sigma ^{2}) }}} and {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{2 \log (1.25/\delta )r^{2}}{\epsilon ^{2}}}}}, and all {{\color{\colorMATH}\ensuremath{\epsilon _{i}, \delta _{i} > 0}}}:

  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d^{\prime}]) = d]} \leq  e^{\epsilon _{i}} + \delta _{i}
  \vspace*{-1em}\end{gather*}\endgroup 
 \endgroup 
\end{theorem}

\begin{proof}
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  By the assumption, {{\color{\colorMATH}\ensuremath{ \| g(\gamma ) - g(\gamma [i\mapsto d])\| _{2} = \Delta _{2}g \leq  r }}}. The conclusion follows by Dwork and Roth, Theorem A.1. \note{do we need to worry about {{\color{\colorMATH}\ensuremath{\bot }}}?}

  \endgroup 
\end{proof}

\begin{theorem}[Advanced composition]
  \label{thm:adv_comp}
  
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  If {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[g(\gamma ) = d_{1}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[g(\gamma [i\mapsto d_{2}]) = d_{1}]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}, then for all {{\color{\colorMATH}\ensuremath{\delta ^{\prime} > 0}}}:

  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[{{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(k, g(\gamma ), d_{3}) = d_{4}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[{{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(k, g(\gamma [i\mapsto d_{2}]), d_{3}) = d_{4}]} \leq  e^{2\epsilon _{i}\sqrt {2n\log (1/\delta ^{\prime})}} + \delta ^{\prime}+n\delta _{i}
  \vspace*{-1em}\end{gather*}\endgroup 

  Where {{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}}}} is defined as:
  
  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(0, \underline{\hspace{0.66em}\vspace*{5ex}}, d) \triangleq  d
  \cr  {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, g, d) \triangleq  {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n-1, g, g(d))
  \vspace*{-1em}\end{gather*}\endgroup 
 \endgroup 
\end{theorem}

\begin{proof}
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  Define a family of mechanisms {{\color{\colorMATH}\ensuremath{ {\mathcal{F}} = \{g\} }}}. By the assumption, each mechanism {{\color{\colorMATH}\ensuremath{ {\mathcal{M}} \in  {\mathcal{F}} }}} satisfies {{\color{\colorMATH}\ensuremath{ (\epsilon _{i}, \delta _{i}) }}}-differential privacy for each {{\color{\colorMATH}\ensuremath{i}}}. The starting value {{\color{\colorMATH}\ensuremath{ d }}} is considered public, and therefore auxiliary information; we define {{\color{\colorMATH}\ensuremath{w_{j} = d}}} for each {{\color{\colorMATH}\ensuremath{j \in  1,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},n}}}. Since the class of mechanisms {{\color{\colorMATH}\ensuremath{ {\mathcal{F}} }}} satisfies {{\color{\colorMATH}\ensuremath{ (\epsilon _{i}, \delta _{i}) }}}-differential privacy, by Dwork and Roth, Theorem 3.20, this class satisfies {{\color{\colorMATH}\ensuremath{(2\epsilon _{i}\sqrt {2n\log (1/\delta ^{\prime})}, \delta ^{\prime}+n\delta _{i})}}}-differential privacy under {{\color{\colorMATH}\ensuremath{n}}}-fold adaptive composition.

  Next, we show that {{\color{\colorMATH}\ensuremath{ {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, g, d) }}} is an instance of {{\color{\colorMATH}\ensuremath{n}}}-fold adaptive composition of the class of mechanisms {{\color{\colorMATH}\ensuremath{{\mathcal{F}}}}}. Pick an adversary {{\color{\colorMATH}\ensuremath{A}}} which, at each iteration {{\color{\colorMATH}\ensuremath{j \in  1,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},n}}}, runs {{\color{\colorMATH}\ensuremath{{\mathcal{M}} \in  {\mathcal{F}}}}} with the output of the previous iteration (using {{\color{\colorMATH}\ensuremath{d}}} as the input for the first iteration). This is exactly the definition of {{\color{\colorMATH}\ensuremath{ {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, g, d) }}}. \note{do we have to worry about {{\color{\colorMATH}\ensuremath{\bot }}}s or the {{\color{\colorMATH}\ensuremath{i}}}s?}
  \endgroup 
\end{proof}

\begin{theorem}
  \label{thm:let}

  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} {{\color{\colorTEXT}\textit{If}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{1}(\gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{1}(\gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime}} + \delta _{i}^{\prime}
  \cr  {{\color{\colorTEXT}\textit{and}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(d^{\prime \prime}, \gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(d^{\prime \prime}, \gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime \prime}
  \cr  {{\color{\colorTEXT}\textit{then}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma ),\gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime} + \delta _{i}^{\prime \prime}
  \vspace*{-1em}\end{gather*}\endgroup 
  \endgroup 
\end{theorem}

\begin{proof}
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  We appeal to Dwork and Roth, Theorem~B.1, which requires two differentially private functions:

  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} T_{1}(D) : D \rightarrow  {\mathcal{C}}_{1}
  \cr  T_{2}(D, s_{1}) : (D, s_{1}) \rightarrow  {\mathcal{C}}_{2}
  \vspace*{-1em}\end{gather*}\endgroup 

  Let {{\color{\colorMATH}\ensuremath{ T_{1} = f_{1} }}} and {{\color{\colorMATH}\ensuremath{ T_{2} = f_{2} }}} (swapping the arguments of {{\color{\colorMATH}\ensuremath{ f_{2} }}}). By Dwork and Roth, Theorem~B.1, if {{\color{\colorMATH}\ensuremath{\gamma }}} and {{\color{\colorMATH}\ensuremath{\gamma [i\mapsto d]}}} are neighbors, for each {{\color{\colorMATH}\ensuremath{i}}} we have that:

  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[(f_{1}(\gamma ), f_{2}(f_{1}(\gamma ),\gamma )) = d^{\prime}]}
  {{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[(f_{1}(\gamma [i\mapsto d]), f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d])) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime} + \delta _{i}^{\prime \prime}
  \vspace*{-1em}\end{gather*}\endgroup 

  i.e. releasing the tuple containing the results of both functions yields {{\color{\colorMATH}\ensuremath{ (e^{\epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}}, \delta _{i}^{\prime} + \delta _{i}^{\prime \prime} ) }}}-differential privacy.

  By Dwork and Roth, Proposition 2.1 (post-processing), we can release just the second element of this tuple with the same privacy cost (which is what we want to show).
  \endgroup 
\end{proof}



\section{Proofs}

\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \Gamma \vdash \underline{\hspace{0.66em}\vspace*{5ex}}\mathrel{:}\tau \rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{exp}}}} \rightarrow  \llbracket \Gamma  \vdash  \tau \rrbracket  \endgroup}\endgroup \end{tabularx}
\cr  \llbracket  \Gamma  \vdash  x \mathrel{:} \tau  \rrbracket  \triangleq  {.}\hspace{-1pt}{.}\hspace{-1pt}{.}
\cr  \llbracket  \{ x_{1} \mathrel{:}_{r_{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{r_{n}} \tau _{n}\}  \vdash  x_{i} \mathrel{:} \tau  \rrbracket  \triangleq  f = \lambda  \langle x_{1}, ..., x_{n}\rangle  . x_{i}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{to show:}}}\hspace*{0.33em}x_{j} \ominus _{j} x_{j}^{\prime} \leq  1 \implies   f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \leq  r_{j}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{case 1:}}}\hspace*{0.33em}j \neq  i: {{\color{\colorTEXT}\textit{we have}}}\hspace*{0.33em}f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) = x_{i} \ominus _{j} x_{i} \leq  0 \leq  r_{j}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{case 2:}}}\hspace*{0.33em}j = i: {{\color{\colorTEXT}\textit{we have}}}\hspace*{0.33em}f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) = x_{i} \ominus _{j} x_{i}^{\prime} \leq  1 \leq  r_{j}
\cr  \llbracket  \{ x_{1} \mathrel{:}_{r_{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{r_{n}} \tau _{n}\}  \vdash  \lambda  x. e \mathrel{:} \tau _{1} \multimap _{s} \tau _{2} \rrbracket  \triangleq  f = \lambda  \langle x_{1}, ..., x_{n}\rangle  . \lambda  x . f^{\prime}(x_{1}, ..., x_{n}, x)
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 

\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \Gamma \vdash \underline{\hspace{0.66em}\vspace*{5ex}}\mathrel{:}\tau \rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{exp}}}} \rightarrow  \llbracket \Gamma  \vdash  \tau \rrbracket  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begin{itemize}[leftmargin=*,label=\textbf{-
}]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{ e = {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup }}}}
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma ^{\prime}}{\infty {\otimes }{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma ^{\dagger }}}}\endgroup }} \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup } \mathrel{:} \tau \rrbracket  \triangleq  f}}}
%   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma  \vdash  e \mathrel{:} \tau  }}}\endgroup }}}}
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma \in \llbracket \Gamma ^{\prime}\rrbracket ,d\in \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma [i] \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = x]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
   \\\noindent  we have that for all {{\color{\colorMATH}\ensuremath{i}}}, {{\color{\colorMATH}\ensuremath{\gamma [i] = \infty }}}, so the result holds trivially
   
% \noindent  Case {{\color{\colorMATH}\ensuremath{e = x_{i}}}}: \note{do we still have a variable rule?}
%    \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma  = \Gamma ^{\prime}\oplus \{ x_{i}\mathrel{:}_{\infty }\} }{\{ x_{1} \mathrel{:}_{\epsilon _{1},\delta _{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.}, x_{i} \mathrel{:} _{\infty } \tau _{i},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{\epsilon _{n},\delta _{n}} \tau _{n}\} } \vdash  x_{i} \mathrel{:} \tau  \rrbracket  \triangleq  f}}}
%    \\\noindent  where {{\color{\colorMATH}\ensuremath{f \triangleq  \lambda \gamma .\hspace*{0.33em} \gamma [i]}}}.
%    \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma \in \llbracket \Gamma \rrbracket ,d\in \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma [i] \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = x]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
%       \begin{itemize}[leftmargin=*,label=\textbf{*
%       }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{j\neq i}}}:
%          \\\noindent  we have {{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = x] = {{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = x]}}}
%          \\\noindent  so for {{\color{\colorMATH}\ensuremath{\epsilon _{j} \geq  0}}} and {{\color{\colorMATH}\ensuremath{\delta _{j} \geq  0}}} the result holds
%          
%       \item  \noindent  Case {{\color{\colorMATH}\ensuremath{j=i}}}:
%          \\\noindent  {{\color{\colorMATH}\ensuremath{e^{\infty } = \infty }}} so the result holds trivially
%          
%       \end{itemize}
%    
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{ e = \lambda x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}.e }}}
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma ^{\prime}}{\infty {\otimes }\Gamma } \vdash  \lambda x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}.e \mathrel{:} [\tau _{1}@_{\epsilon _{1},\delta _{1}},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\tau _{n}@_{\epsilon _{n},\delta _{n}}] \multimap ^{*} \tau  \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{ f \triangleq  \lambda  \gamma  .\hspace*{0.33em} \lambda  d_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},d_{n} .\hspace*{0.33em} f^{\prime}(\gamma  + [x_{1} \mapsto  d_{1}, {.}\hspace{-1pt}{.}\hspace{-1pt}{.}, x_{n} \mapsto  d_{n}] ) }}}
   \\\noindent  (1) to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma \in \llbracket \Gamma ^{\prime}\rrbracket ,d\in \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma [i] \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = x]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
   \\\noindent  But we have that for all {{\color{\colorMATH}\ensuremath{i}}}, {{\color{\colorMATH}\ensuremath{\epsilon _{i} = \delta _{i} = \infty }}}, so this is trivial
   \\\noindent  (2) to show: {{\color{\colorMATH}\ensuremath{ \forall  (d_{1}, {.}\hspace{-1pt}{.}\hspace{-1pt}{.}, d_{n}) \in  \llbracket \tau _{1} \times  {.}\hspace{-1pt}{.}\hspace{-1pt}{.} \times  \tau _{n}\rrbracket , d_{i}^{\prime} \in  \llbracket \tau _{i}\rrbracket  .\hspace*{0.33em} d_{i} \ominus _{i} d_{i}^{\prime} \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma )(d_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},d_{i},{.}\hspace{-1pt}{.}\hspace{-1pt}{.}d_{n}) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma )(d_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},d_{i}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.}d_{n}) = x]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
   \\\noindent  Follows directly from inductive hypothesis
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = \{ x\mathrel{:}_{\infty }[\tau _{1}@s_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\tau _{n}@s_{n}]\multimap ^{*}\tau ,x_{1}\mathrel{:}_{s_{1}}\tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}\mathrel{:}_{s_{n}}\tau _{n}\}  \vdash  x(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \mathrel{:} \tau }}}
   \\\noindent  {{\color{\colorMATH}\ensuremath{ \llbracket  \overbracketarg {\Gamma ^{\prime}}{\{ x\mathrel{:}_{\infty }[\tau _{1}@s_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\tau _{n}@s_{n}]\multimap ^{*}\tau ,x_{1}\mathrel{:}_{s_{1}}\tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}\mathrel{:}_{s_{n}}\tau _{n}\} } \vdash  x(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \mathrel{:} \tau  \rrbracket  \triangleq  f }}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{ f \triangleq  \lambda  \gamma  .\hspace*{0.33em} \gamma [x](\gamma [x_{1}], {.}\hspace{-1pt}{.}\hspace{-1pt}{.}, \gamma [x_{n}]) }}}
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma \in \llbracket \Gamma ^{\prime}\rrbracket ,d\in \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma [i] \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = x]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = x]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
      \begin{itemize}[leftmargin=*,label=\textbf{*
      }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{x_{i} = x}}}:
         \\\noindent  {{\color{\colorMATH}\ensuremath{ \epsilon _{i} = \infty  }}} so the result holds trivially
         
       \item  \noindent  Case {{\color{\colorMATH}\ensuremath{x_{i} \in  \{ x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}\} }}}:
         \\\noindent  follows by the definition of {{\color{\colorMATH}\ensuremath{ \multimap ^{*} }}} where {{\color{\colorMATH}\ensuremath{\epsilon _{i},\delta _{i} = s_{i}}}}
         
      \end{itemize}
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x=e_{1}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}e_{2}}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma ^{\prime}}{\Gamma _{1} \oplus  \Gamma _{2}} \vdash  {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x=e_{1}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}e_{2} \mathrel{:} \tau _{2} \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{ f \triangleq  \lambda  \gamma  .\hspace*{0.33em} f_{2}(f_{1}(\gamma ),\gamma ) }}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{1} \in  \llbracket  \Gamma _{1} \vdash  e_{1} \mathrel{:} \tau _{1} \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{1}(\gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{1}(\gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime}} + \delta _{i}^{\prime}}}} (where {{\color{\colorMATH}\ensuremath{\epsilon _{i}^{\prime},\delta _{i}^{\prime} \in  \Gamma _{1}}}})
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{2} \in  \llbracket  \{ x \mathrel{:}_{\infty }\tau _{1}\} \uplus \Gamma _{2} \vdash  e_{2} \mathrel{:} \tau _{2} \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d^{\prime} \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(d,\gamma ) = d^{\prime \prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(d,\gamma [i\mapsto d^{\prime}]) = d^{\prime \prime}]} \leq  e^{\epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime \prime}}}} (where {{\color{\colorMATH}\ensuremath{\epsilon _{i}^{\prime \prime},\delta _{i}^{\prime \prime} \in  \Gamma _{2}}}})
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma ),\gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}} + \delta _{i} = e^{\epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime} + \delta _{i}^{\prime \prime}}}}
   \\\noindent  this follows directly by Theorem~\ref{thm:let} %, {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma ),\gamma ) = d^{\prime}]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d]) = d^{\prime}]} \leq  e^{\epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}} + \delta _{i}^{\prime} + \delta _{i}^{\prime \prime}}}}
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\epsilon }}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\delta }}}}{=}x_{1},x_{2},x_{3}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e}}}\endgroup }]}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma ^{\prime}}{(\epsilon ,\delta ){\otimes } {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma ^{\dagger } }}}\endgroup } \oplus  \{ x_{1} \mathrel{:}_{\infty } {{\color{\colorSYNTAX}\texttt{real}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r}}}\endgroup }],x_{2} \mathrel{:}_{\infty } {{\color{\colorSYNTAX}\texttt{real}}}[\epsilon ],x_{3} \mathrel{:}_{\infty } {{\color{\colorSYNTAX}\texttt{real}}}[\delta ]\} } \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\epsilon }}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\delta }}}}{=}e_{1},e_{2},e_{3}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ e_{4} }}}\endgroup }] \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{f \triangleq  \lambda  \gamma  .\hspace*{0.33em} f^{\prime}(\gamma ) + {\mathcal{N}}(0, \sigma ^{2})}}}
   % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{1} \in  \llbracket  \Gamma _{1} \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[r] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{1}(\gamma ) = \lfloor r\rfloor _{{\mathcal{D}}}}}}
   % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{2} \in  \llbracket  \Gamma _{2} \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\epsilon ] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{2}(\gamma ) = \lfloor \epsilon \rfloor _{{\mathcal{D}}}}}}
   % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{3} \in  \llbracket  \Gamma _{3} \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\delta ] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{3}(\gamma ) = \lfloor \delta \rfloor _{{\mathcal{D}}}}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f^{\prime} \in  \llbracket  {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{r{\otimes } \Gamma ^{\dagger } \vdash  e \mathrel{:} {\mathcal{S}}_{r^{\prime}}({{\color{\colorSYNTAX}\texttt{real}}}) }}}\endgroup } \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma  }}}\endgroup }\rrbracket ,d \in  \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma (i) \ominus _{i} d \leq  1 \implies   |f^{\prime}(\gamma ) - f^{\prime}(\gamma [i\mapsto d])| \leq  r}}}
   \\\noindent  where: {{\color{\colorMATH}\ensuremath{\sigma ^{2} = \frac{2 \log (1.25/\delta )r^{2}}{\epsilon ^{2}}}}}
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma ^{\prime}\rrbracket ,d \in  \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma (i) \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
   \\\noindent  \begin{itemize}[leftmargin=*,label=\textbf{*
      }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{x_{i} \in  \{  x_{1}, x_{2}, x_{3} \} }}}
         \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\infty } + \infty }}} which is trivial
         
      \item  \noindent  Case {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta ){\otimes } {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma ^{\dagger } }}}\endgroup }[i] \neq  \bot }}} and {{\color{\colorMATH}\ensuremath{ x_{i} \notin  \{  x_{1}, x_{2}, x_{3} \} }}}
         \\\noindent  we have that {{\color{\colorMATH}\ensuremath{ ((\epsilon ,\delta ){\otimes } {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma ^{\dagger } }}}\endgroup })[i] = \epsilon , \delta }}}, so {{\color{\colorMATH}\ensuremath{ \epsilon _{i} = \epsilon  }}} and {{\color{\colorMATH}\ensuremath{ \delta _{i} = \delta  }}}
         \\\noindent  by Theorem~\ref{thm:gauss}, {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon } + \delta }}}
         % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{L_{2}}}} sensitivity of {{\color{\colorMATH}\ensuremath{f_{4}}}} {w.r.t.} {{\color{\colorMATH}\ensuremath{x_{i}}}} is bounded by {{\color{\colorMATH}\ensuremath{r}}}
         % \\\noindent  by Gaussian mech.: {{\color{\colorMATH}\ensuremath{f_{4}(\gamma ) + {\mathcal{N}}(0, \sigma ^{2})}}} provides {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy for {{\color{\colorMATH}\ensuremath{x_{i}}}}
         % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{\epsilon _{i} = \epsilon }}} and {{\color{\colorMATH}\ensuremath{\delta _{i} = \delta }}} for all {{\color{\colorMATH}\ensuremath{i}}} such that {{\color{\colorMATH}\ensuremath{\Gamma _{4}[i] \neq  \bot }}}
         % \\\noindent  by defn. differential privacy: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
         
      % \item  \noindent  Case {{\color{\colorMATH}\ensuremath{\Gamma _{4}[i] = \bot }}} and {{\color{\colorMATH}\ensuremath{(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})[i] = \bot }}}
      %    \\\noindent  nothing to show in this case
      %    
      % \item  \noindent  Case {{\color{\colorMATH}\ensuremath{(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})[i] \neq  \bot }}}
      %    \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\infty } + \infty }}} which is trivial
      %    
      \end{itemize}
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = {{\color{\colorSYNTAX}\texttt{loop}}}[{{\color{\colorSYNTAX}\texttt{n}}},{{\color{\colorSYNTAX}\texttt{i}}}=x_{1},x_{2}][x.e]}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma ^{\prime}}{(2\epsilon \sqrt {2n\log (1/\delta ^{\prime})},\delta ^{\prime}+n\delta ){\otimes }\Gamma ^{\dagger } \oplus  \{ x_{1} \mathrel{:}_{\infty } {{\color{\colorSYNTAX}\texttt{nat}}}[n], x_{2} \mathrel{:}_{\infty } \tau \} } \vdash 
       {{\color{\colorSYNTAX}\texttt{loop}}}[{{\color{\colorSYNTAX}\texttt{n}}},{{\color{\colorSYNTAX}\texttt{i}}}=x_{1},x_{2}][x.e] \mathrel{:} \tau  \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{f \triangleq  \lambda  \gamma  .\hspace*{0.33em} {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(x_{1}, f^{\prime}(\gamma ), x_{2})}}}
   \\\noindent  \hspace*{1.00em}\hspace*{1.00em}\hspace*{1.00em} {{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(0, \underline{\hspace{0.66em}\vspace*{5ex}}, d) \triangleq  d}}}
   \\\noindent  \hspace*{1.00em}\hspace*{1.00em}\hspace*{1.00em} {{\color{\colorMATH}\ensuremath{{{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, g, d) \triangleq  {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n-1, g, g(d))}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f^{\prime} \in  \llbracket  (\epsilon ,\delta ){\otimes }\Gamma ^{\dagger } \uplus  \{ x \mathrel{:}_{\infty } \tau \}  \vdash  e \mathrel{:} \tau  \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket ,d \in  \llbracket \tau _{i}\rrbracket  .\hspace*{0.33em} \gamma (i) \ominus _{i} d \leq  1 \implies   \frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon } + \delta }}}
   \\\noindent  \begin{itemize}[leftmargin=*,label=\textbf{*
      }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{x_{i} \in  \{  x_{1}, x_{2} \} }}}
         \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\infty } + \infty }}} which is trivial
         
      \item  \noindent  Case {{\color{\colorMATH}\ensuremath{x_{i} \notin  \{  x_{1}, x_{2} \} }}} and {{\color{\colorMATH}\ensuremath{ \Gamma [i] \neq  \bot }}}
         \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{2\epsilon \sqrt {2n\log (1/\delta ^{\prime})}} + \delta ^{\prime}+n\delta }}}
         \\\noindent  by IH, {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f^{\prime}(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f^{\prime}(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon } + \delta }}}
         %{{\color{\colorMATH}\ensuremath{f_{2}}}} is a mechanism that provides {{\color{\colorMATH}\ensuremath{\epsilon , \delta }}}-differential privacy for {{\color{\colorMATH}\ensuremath{x_{i}}}}
         % \\\noindent  by IH, {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{1}(\gamma ) = \lfloor n\rfloor _{{\mathcal{D}}}}}}
         % \\\noindent  by IH and case condition, {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket  .\hspace*{0.33em} f_{3}(\gamma ) = f_{3}(\gamma [i\mapsto d])}}}
         % \\\noindent  we therefore have that {{\color{\colorMATH}\ensuremath{ f = \lambda  \gamma  .\hspace*{0.33em} {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, f_{2}(\gamma ), v) }}}
         \\\noindent  by Theorem~\ref{thm:adv_comp}, {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{2\epsilon \sqrt {2n\log (1/\delta ^{\prime})}} + \delta ^{\prime}+n\delta }}}
         % \\\noindent  by something, {{\color{\colorMATH}\ensuremath{\lambda  \gamma  .\hspace*{0.33em} {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, f_{2}(\gamma ), v)}}} is an instance of {{\color{\colorMATH}\ensuremath{n}}}-fold adaptive composition for {{\color{\colorMATH}\ensuremath{x_{i}}}}
         % \\\noindent  by D\&R, 3.20, for all {{\color{\colorMATH}\ensuremath{\delta ^{\prime} > 0}}}, {{\color{\colorMATH}\ensuremath{\lambda  \gamma  .\hspace*{0.33em} {{\color{\colorMATH}\ensuremath{\operatorname{iter}}}}(n, f_{2}(\gamma ), v)}}} satisfies {{\color{\colorMATH}\ensuremath{2\epsilon \sqrt {2n\log (1/\delta ^{\prime})},\delta ^{\prime}+n\delta }}}-differential privacy for {{\color{\colorMATH}\ensuremath{x_{i}}}}
         % \\\noindent  by defin. differential privacy: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{2\epsilon \sqrt {2n\log (1/\delta ^{\prime})}} + \delta ^{\prime}+n\delta }}}
         
      \end{itemize}
   
\end{itemize}
\endgroup 

\clearpage

\section{Proofs (R\'enyi Differential Privacy)}

\begin{theorem}[Gaussian mechanism (R\'enyi Differential Privacy)]
  \label{thm:gauss_renyi}
  
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  If {{\color{\colorMATH}\ensuremath{ | g(\gamma ) - g(\gamma [i\mapsto d]) | \leq  r }}}, then for {{\color{\colorMATH}\ensuremath{ f = \lambda  \gamma  .\hspace*{0.33em} g(\gamma ) + {\mathcal{N}}(0, \sigma ^{2}) }}} and {{\color{\colorMATH}\ensuremath{ \sigma ^{2} = \alpha  / (2\epsilon ) }}}, and all {{\color{\colorMATH}\ensuremath{\epsilon  > 0}}}:

  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d^{\prime}])) \leq  \epsilon 
  \vspace*{-1em}\end{gather*}\endgroup 
 \endgroup 
\end{theorem}

\begin{proof}
  By Mironov, Proposition 7, we have that:

  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d^{\prime}])) \leq  \alpha  / (2\sigma ^{2}) = \epsilon 
  \vspace*{-1em}\end{gather*}\endgroup 
  \endgroup 
\end{proof}


\begin{theorem}[Adaptive sequential composition (R\'enyi differential privacy)]
  \label{thm:let_renyi}

  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  \vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} {{\color{\colorTEXT}\textit{If}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{1}(\gamma ) \|  f_{1}(\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime}
  \cr  {{\color{\colorTEXT}\textit{and}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(d^{\prime \prime}, \gamma ) \|  f_{2}(d^{\prime \prime}, \gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime \prime}
  \cr  {{\color{\colorTEXT}\textit{then}}}\hspace*{0.33em}\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(f_{1}(\gamma ),\gamma ) \|  f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime}
  \vspace*{-1em}\end{gather*}\endgroup 
  \endgroup 
\end{theorem}

\begin{proof}
  \begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
  The result follows directly from Mironov, Proposition 1, setting {{\color{\colorMATH}\ensuremath{f = f_{1}}}} and {{\color{\colorMATH}\ensuremath{g = f_{2}}}}.
  \endgroup 
\end{proof}


\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \Gamma \vdash \underline{\hspace{0.66em}\vspace*{5ex}}\mathrel{:}\tau \rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{exp}}}} \rightarrow  \llbracket \Gamma  \vdash  \tau \rrbracket  \endgroup}\endgroup \end{tabularx}
\cr  \llbracket  \Gamma  \vdash  x \mathrel{:} \tau  \rrbracket  \triangleq  {.}\hspace{-1pt}{.}\hspace{-1pt}{.}
\cr  \llbracket  \{ x_{1} \mathrel{:}_{r_{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{r_{n}} \tau _{n}\}  \vdash  x_{i} \mathrel{:} \tau  \rrbracket  \triangleq  f = \lambda  \langle x_{1}, ..., x_{n}\rangle  . x_{i}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{to show:}}}\hspace*{0.33em}x_{j} \ominus _{j} x_{j}^{\prime} \leq  1 \implies   f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \leq  r_{j}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{case 1:}}}\hspace*{0.33em}j \neq  i: {{\color{\colorTEXT}\textit{we have}}}\hspace*{0.33em}f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) = x_{i} \ominus _{j} x_{i} \leq  0 \leq  r_{j}
\cr  \hspace*{1.00em}{{\color{\colorTEXT}\textit{case 2:}}}\hspace*{0.33em}j = i: {{\color{\colorTEXT}\textit{we have}}}\hspace*{0.33em}f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) \ominus _{j} f(x_{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{j}^{\prime},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n}) = x_{i} \ominus _{j} x_{i}^{\prime} \leq  1 \leq  r_{j}
\cr  \llbracket  \{ x_{1} \mathrel{:}_{r_{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{r_{n}} \tau _{n}\}  \vdash  \lambda  x. e \mathrel{:} \tau _{1} \multimap _{s} \tau _{2} \rrbracket  \triangleq  f = \lambda  \langle x_{1}, ..., x_{n}\rangle  . \lambda  x . f^{\prime}(x_{1}, ..., x_{n}, x)
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 

\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \Gamma \vdash \underline{\hspace{0.66em}\vspace*{5ex}}\mathrel{:}\tau \rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{exp}}}} \rightarrow  \llbracket \Gamma  \vdash  \tau \rrbracket  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begin{itemize}[leftmargin=*,label=\textbf{-
}]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = x_{i}}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma  = \Gamma ^{\prime}\oplus \{ x_{i}\mathrel{:}_{\infty }\} }{\{ x_{1} \mathrel{:}_{\alpha ,\epsilon _{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.}, x_{i} \mathrel{:} _{\infty } \tau _{i},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{\alpha ,\epsilon _{n}} \tau _{n}\} } \vdash  x_{i} \mathrel{:} \tau  \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{f \triangleq  \lambda \gamma .\hspace*{0.33em} \gamma [i]}}}.
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma \in \llbracket \Gamma \rrbracket ,d\in \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma [i] \ominus _{i} d \leq  1 \implies   D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d])) \leq  \epsilon _{i} }}}
      \begin{itemize}[leftmargin=*,label=\textbf{*
      }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{j\neq i}}}:
         \\\noindent  we have {{\color{\colorMATH}\ensuremath{D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d])) = 0 }}}
         \\\noindent  so for {{\color{\colorMATH}\ensuremath{\epsilon _{j} \geq  0}}} the result holds
         
      \item  \noindent  Case {{\color{\colorMATH}\ensuremath{j=i}}}:
         \\\noindent  {{\color{\colorMATH}\ensuremath{\epsilon  = \infty }}} so the result holds trivially
         
      \end{itemize}
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x=e_{1}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}e_{2}}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma =\Gamma _{1} \oplus  \Gamma _{2}}{\{ x_{1} \mathrel{:}_{\alpha ,\epsilon _{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{\alpha ,\epsilon _{n}} \tau _{n}\} } \vdash  {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x=e_{1}\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}e_{2} \mathrel{:} \tau _{2} \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{ f \triangleq  \lambda  \gamma  .\hspace*{0.33em} f_{2}(f_{1}(\gamma ),\gamma ) }}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{1} \in  \llbracket  \Gamma _{1} \vdash  e_{1} \mathrel{:} \tau _{1} \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{1}(\gamma ) \|  f_{1}(\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime} }}} (where {{\color{\colorMATH}\ensuremath{\epsilon _{i}^{\prime} \in  \Gamma _{1}}}})
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{2} \in  \llbracket  \{ x \mathrel{:}_{\infty }\tau _{1}\} \uplus \Gamma _{2} \vdash  e_{2} \mathrel{:} \tau _{2} \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d^{\prime} \leq  1 \implies  D_{\alpha }(f_{2}(d,\gamma ) \|  f_{2}(d,\gamma [i\mapsto d^{\prime}])) \leq  \epsilon _{i}^{\prime \prime} }}} (where {{\color{\colorMATH}\ensuremath{\epsilon _{i}^{\prime \prime} \in  \Gamma _{2}}}})
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(f_{1}(\gamma ),\gamma ) \|  f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d])) \leq  \epsilon _{i} = \epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime} }}}
   \\\noindent  by Theorem~\ref{thm:let_renyi}, {{\color{\colorMATH}\ensuremath{\gamma [i] \ominus _{i} d \leq  1 \implies  D_{\alpha }(f_{2}(f_{1}(\gamma ),\gamma ) \|  f_{2}(f_{1}(\gamma [i\mapsto d]),\gamma [i\mapsto d])) \leq  \epsilon _{i}^{\prime} + \epsilon _{i}^{\prime \prime} }}} 
   
\item  \noindent  Case {{\color{\colorMATH}\ensuremath{e = {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\alpha }}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\epsilon }}}}{=}e_{1},e_{2},e_{3}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{e_{4}}}}\endgroup }]}}}:
   \\\noindent  {{\color{\colorMATH}\ensuremath{\llbracket  \overbracketarg {\Gamma =\infty {\otimes }(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})\oplus (\alpha , \epsilon ){\otimes }{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{\Gamma _{4}^{\dagger }}}}\endgroup }}{\{ x_{1} \mathrel{:}_{\alpha ,\epsilon _{1}} \tau _{1},{.}\hspace{-1pt}{.}\hspace{-1pt}{.},x_{n} \mathrel{:}_{\alpha ,\epsilon _{n}} \tau _{n}\} } \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\alpha }}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\epsilon }}}}{=}e_{1},e_{2},e_{3}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ e_{4} }}}\endgroup }] \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} \rrbracket  \triangleq  f}}}
   \\\noindent  where {{\color{\colorMATH}\ensuremath{f \triangleq  \lambda  \gamma  .\hspace*{0.33em} f_{4}(\gamma ) + {\mathcal{N}}(0, \sigma ^{2})}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{1} \in  \llbracket  \Gamma _{1} \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[r] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{1}(\gamma ) = \lfloor r\rfloor _{{\mathcal{D}}}}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{2} \in  \llbracket  \Gamma _{2} \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\alpha ] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{2}(\gamma ) = \lfloor \alpha \rfloor _{{\mathcal{D}}}}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{3} \in  \llbracket  \Gamma _{3} \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\epsilon ] \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket . f_{3}(\gamma ) = \lfloor \epsilon \rfloor _{{\mathcal{D}}}}}}
   \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{f_{4} \in  \llbracket  r {\otimes } \Gamma _{4} \vdash  e_{4} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} \rrbracket }}} and {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket ,d \in  \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma (i) \ominus _{i} d \leq  1 \implies   |f_{4}(\gamma ) - f_{4}(\gamma [i\mapsto d])| \leq  r}}}
   \\\noindent  where: {{\color{\colorMATH}\ensuremath{ \sigma ^{2} = \alpha  / (2\epsilon ) }}}
   \\\noindent  to show: {{\color{\colorMATH}\ensuremath{\forall  \gamma  \in  \llbracket \Gamma \rrbracket ,d \in  \llbracket \tau _{i}\rrbracket .\hspace*{0.33em} \gamma (i) \ominus _{i} d \leq  1 \implies   D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d])) \leq  \epsilon _{i} }}}
   \\\noindent  \begin{itemize}[leftmargin=*,label=\textbf{*
      }]\item  \noindent  Case {{\color{\colorMATH}\ensuremath{\Gamma _{4}[i] \neq  \bot }}} and {{\color{\colorMATH}\ensuremath{(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})[i] = \bot }}}
         \\\noindent  by Theorem~\ref{thm:gauss_renyi}, {{\color{\colorMATH}\ensuremath{D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d])) \leq  \epsilon }}}
         % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{L_{2}}}} sensitivity of {{\color{\colorMATH}\ensuremath{f_{4}}}} {w.r.t.} {{\color{\colorMATH}\ensuremath{x_{i}}}} is bounded by {{\color{\colorMATH}\ensuremath{r}}}
         % \\\noindent  by Gaussian mech.: {{\color{\colorMATH}\ensuremath{f_{4}(\gamma ) + {\mathcal{N}}(0, \sigma ^{2})}}} provides {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy for {{\color{\colorMATH}\ensuremath{x_{i}}}}
         % \\\noindent  by IH: {{\color{\colorMATH}\ensuremath{\epsilon _{i} = \epsilon }}} and {{\color{\colorMATH}\ensuremath{\delta _{i} = \delta }}} for all {{\color{\colorMATH}\ensuremath{i}}} such that {{\color{\colorMATH}\ensuremath{\Gamma _{4}[i] \neq  \bot }}}
         % \\\noindent  by defn. differential privacy: {{\color{\colorMATH}\ensuremath{\frac{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma ) = d]}{{{\color{\colorMATH}\ensuremath{\operatorname{Pr}}}}[f(\gamma [i\mapsto d]) = d]} \leq  e^{\epsilon _{i}} + \delta _{i}}}}
         
      \item  \noindent  Case {{\color{\colorMATH}\ensuremath{\Gamma _{4}[i] = \bot }}} and {{\color{\colorMATH}\ensuremath{(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})[i] = \bot }}}
         \\\noindent  nothing to show in this case
         
      \item  \noindent  Case {{\color{\colorMATH}\ensuremath{(\Gamma _{1}\oplus \Gamma _{2}\oplus \Gamma _{3})[i] \neq  \bot }}}
         \\\noindent  to show: {{\color{\colorMATH}\ensuremath{D_{\alpha }(f(\gamma ) \|  f(\gamma [i\mapsto d])) \leq  \infty }}} which is trivial
         
      \end{itemize}
   
\end{itemize}
\endgroup 


==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}


The initial definition of differential privacy is due to Cynthia Dwork~\cite{dworkdifferential2006, dwork2006calibrating, dwork2008differential}. The book by Dwork and Roth~\cite{privacybook} provides an excellent overview of techniques in differential privacy.

\paragraph{Systems for Differential Privacy.}
Several systems exist for enforcing differential privacy on database-style queries. The first of these, Privacy Integrated Queries (PINQ)~\cite{mcsherry2009privacy}, answers database queries and implements the Laplace mechanism with a measure of global sensitivity. The calculus used in PINQ can be viewed as a privacy type system for such queries.
%Weighted PINQ~\cite{proserpio2014calibrating} extends PINQ to weighted datasets.

Other systems include FLEX~\cite{johnson2018towards, es_paper_arxiv}, for SQL queries; Airavat~\cite{roy2010airavat}, for MapReduce programs; %Fuzz~\cite{gaboardi2013linear,haeberlen2011differential} enforces differential privacy for functional programs, using the Laplace mechanism in an approach similar to PINQ.
DJoin~\cite{narayan2012djoin} for queries over distributed datasets; and GUPT~\cite{mohan2012gupt}, which implements the Sample \& Aggregate framework for Python programs.
%None supports machine learning tasks.


\paragraph{Differentially private machine learning.}
A large body of work exists on differentially private convex empirical risk minimization (ERM), from which we draw the algorithms considered in this paper. The first algorithms proposed were output perturbation and objective perturbation~\cite{cms11}. The private SGD algorithm was first proposed by Song et al.~\cite{SCS}, with improved risk bounds due to Bassily et al.~\cite{bst14}. More recently, an improved versions of output perturbation~\cite{PSGD}
% and objective perturbation~\cite{dpml}
has been proposed.
%
The high-dimensional setting has also been studied~\cite{KST12, ST13}, and the private Frank-Wolfe algorithm we consider in this paper is due to Talwar et al.~\cite{TTZ15a}.

%Differentially private convex optimization has also been explored in the online setting~\cite{JKT12, DJW13, ST13b}, for high-dimensional kernel learning~\cite{JT13}, and in regression analysis~\cite{Z12, W15}.

In the non-convex case, achieving differential privacy is more challenging. The first approach for deep learning was proposed by Shokri and Shmatikov~\cite{SS15}, and employed a private SGD algorithm in combination with clamping of the gradient. More recently, Talwar et al.~\cite{DPDL} improved on this result by introducing the \emph{moments accountant}, which yields tighter bounds on the privacy loss. As we have shown, \system is capable of reproducing both results automatically.
%Recent work by Papernot et al.~\cite{papernot2016semi} proposes an approach for deep learning that trains many \emph{non-private} models, then uses them to train a single differentially private model.
%
%These approaches are complementary to our work, and could be integrated into \system to enable learning pipelines that employ deep learning.


%SGD
%The first differentially private version was proposed by Chaudhuri et al.~\cite{cms11} and refined by . The version we present here, with improved privacy bounds via the moments accountant~\cite{dpdl}, is due to Thakkar et al.~\cite{dpml}.

% Moments accountant
% Advanced composition can also be used with $(\epsilon, \delta)$-differentially private mechanisms, such as the Gaussian mechanism, but it provides looser bounds in this case. For the Gaussian mechanism, the moments accountant provides an improvement of $\sqrt{\ln(\frac{k}{\delta})}$ over the advanced composition theorem, which can be significant for iterative algorithms. For $\epsilon$-differentially private mechanisms, such as the exponential mechanism, the advanced composition theorem provides the best known bound.

\paragraph{Language-based approaches.}
Language-based approaches for differential privacy fall into two categories: approaches based on type systems, and those based on relational verification. Barthe et al.~\cite{barthe2016programming} provide a survey. The type-system based approaches are most related to our work, but relational verification approaches have also received considerable attention in recent years~\cite{barthe2016proving, barthe2016advanced, barthe2013beyond, barthe2013probabilistic, sato2016approximate}.

\input{experiment_results}

Approaches based on type systems began with \fuzz~\cite{reed2010distance}, which uses linear types to track sensitivity. \dfuzz~\cite{dfuzz,dfuzz-impl} adds dependent types to allow for more expressive sensitivity annotations. Winograd-Cort et al.~\cite{winograd2017framework} add a runtime component to \fuzz to provide {{\color{\colorMATH}\ensuremath{(\epsilon , \delta )}}}-differential privacy for iterative algorithms. Our work builds on \fuzz and \dfuzz to provide a static guarantees for variants other than {{\color{\colorMATH}\ensuremath{(\epsilon ,0)}}}-differential privacy.

% The key property preserved by these type systems metric preservation; recent work by Azevedo de Amorim et al.~\cite{azevedo2017semantic} studies this property in detail.
Recent work has made considerable progress in proving differential privacy for
low-level mechanisms. The approach used in
\textsf{HOARe$^2$}~\cite{barthe2015higher} uses refinement types;
LightDP~\cite{zhang2017lightdp} has a relational type system; and Albarghouthi
and Hsu~\cite{albarghouthi2017synthesizing} build on LightDP to prove more
expressive algorithms. All three are capable of proving {{\color{\colorMATH}\ensuremath{(\epsilon , \delta )}}}-differentially
privacy for algorithms, but do not focus on automation. These tools are
complementary to our work: they would enable mechanizing the privacy proofs for
the built-in mechanisms \system provides.


%Relational program logics have also been used to prove differential privacy for \cite{barthe2016proving, barthe2016advanced, barthe2013beyond, barthe2013probabilistic, sato2016approximate}

\begin{comment}
\subsection{Limitations of the Path Construction}
\label{sec:path_construction}

\paragraph{Loose bounds for multiple variables.} Consider the following program:

\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} x \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{1}, \delta _{1}][d_{1}]
\cr  y \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{2}, \delta _{2}][d_{2}]
\vspace*{-1em}\end{gather*}\endgroup 

This program provides {{\color{\colorMATH}\ensuremath{(\epsilon _{1}, \delta _{1})}}}-differential privacy for {{\color{\colorMATH}\ensuremath{d_{1}}}} and {{\color{\colorMATH}\ensuremath{(\epsilon _{2}, \delta _{2})}}}-differential privacy for {{\color{\colorMATH}\ensuremath{d_{2}}}}. However, Arthur's system will produce the following judgment: 

\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} d_{1} \mathrel{:}_{1} {\mathbb{R}}, d_{2} \mathrel{:}_{1} {\mathbb{R}} \vdash 
\cr  \hspace*{1.00em} \hspace*{1.00em} x \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{1}, \delta _{1}][d_{1}]
\cr  \hspace*{1.00em} \hspace*{1.00em} y \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{2}, \delta _{2}][d_{2}]
\cr  \mathrel{:} \bigcirc _{\epsilon _{1}+\epsilon _{2}, \delta _{1}+\delta _{2}} {\mathbb{R}}
\vspace*{-1em}\end{gather*}\endgroup 

implying {{\color{\colorMATH}\ensuremath{(\epsilon _{1}+\epsilon _{2}, \delta _{1}+\delta _{2})}}}-differential privacy for \emph{both} {{\color{\colorMATH}\ensuremath{d_{1}}}} and {{\color{\colorMATH}\ensuremath{d_{2}}}}. It's not clear how to rewrite the program to achieve the standard bounds.

\paragraph{Impossible to avoid group privacy.} Consider a small change to the above program and the corresponding judgment:

\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} d_{1} \mathrel{:}_{2} {\mathbb{R}} \vdash 
\cr  \hspace*{1.00em} \hspace*{1.00em} x \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{1}, \delta _{1}][d_{1}]
\cr  \hspace*{1.00em} \hspace*{1.00em} y \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon _{2}, \delta _{2}][d_{1}]
\cr  \mathrel{:} \bigcirc _{\epsilon _{1}+\epsilon _{2}, \delta _{1}+\delta _{2}} {\mathbb{R}}
\vspace*{-1em}\end{gather*}\endgroup 

This program uses {{\color{\colorMATH}\ensuremath{d_{1}}}} twice. The interpretation of this type in Arthur's system is via group privacy: the program provides {{\color{\colorMATH}\ensuremath{(2(\epsilon _{1}+\epsilon _{2}), (1 + e^{\epsilon _{1}})\delta _{1} + (1 + e^{\epsilon _{2}})\delta _{2})}}}-differential privacy. This is significantly looser than the standard bound via composition of {{\color{\colorMATH}\ensuremath{(\epsilon _{1}+\epsilon _{2}, \delta _{1}+\delta _{2})}}}-differential privacy, and it's not clear how to rewrite the program to avoid the use of group privacy.

\paragraph{Impossible to specify sensitivity other than 1.} Consider the judgment for a program that is 2-sensitive in a single input:

\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*} d \mathrel{:}_{2} {\mathbb{R}} \vdash  x \leftarrow  {{\color{\colorSYNTAX}\texttt{gauss}}}[\epsilon , \delta ][d + d] \mathrel{:} \bigcirc _{\epsilon , \delta } {\mathbb{R}}
\vspace*{-1em}\end{gather*}\endgroup 

As above, the interpretation is via group privacy, yielding {{\color{\colorMATH}\ensuremath{(2\epsilon , (1 + e^{\epsilon })\delta )}}}-differential privacy. As normally defined, the scale of the noise added by the Gaussian mechanism depends on the sensitivity of its argument; as defined in Arthur's system, sensitivities other than 1 can neither be inferred nor specified by the programmer. There is therefore no way to rewrite this program to use the Gaussian mechanism in the standard way, and avoid the use of group privacy.

Moreover, it's not clear how sensitivity could be added to the system. \note{Ask Arthur whether sensitivity could be added to {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{gauss}}}}}} or {{\color{\colorMATH}\ensuremath{\bigcirc }}}.}

\paragraph{Sensitivity is not interchangeable with {{\color{\colorMATH}\ensuremath{\epsilon }}}.} The same issues crop up in the previous systems, \emph{Fuzz} and \emph{DFuzz}, which support only pure {{\color{\colorMATH}\ensuremath{\epsilon }}}-differential privacy. However, these issues can safely be ignored in the context of pure {{\color{\colorMATH}\ensuremath{\epsilon }}}-differential privacy, for two reasons. First, sensitivity and {{\color{\colorMATH}\ensuremath{\epsilon }}} are interchangeable: the Laplace mechanism for sensitivity {{\color{\colorMATH}\ensuremath{\Delta f}}} and privacy parameter {{\color{\colorMATH}\ensuremath{\epsilon }}} is equivalent to the Laplace mechanism for sensitivity {{\color{\colorMATH}\ensuremath{1}}} and privacy parameter {{\color{\colorMATH}\ensuremath{\epsilon  / \Delta f}}}. This is not the case for the Gaussian mechanism---sensitivity cannot be recovered by tweaking the other parameters. Second, group privacy for pure {{\color{\colorMATH}\ensuremath{\epsilon }}}-differential privacy allows linear scaling of the privacy guarantee---so the privacy cost via group privacy of an example like the last one above can be viewed as equivalent to the privacy cost via correctly setting sensitivity. This is not the case for {{\color{\colorMATH}\ensuremath{(\epsilon ,\delta )}}}-differential privacy---in that context, privacy does not scale linearly in the size of the group, and group privacy yields \emph{worse} bounds on privacy cost than setting sensitivity.

\paragraph{Closures are problematic: impossible to add sampling.} 
\end{comment}


==> renyi_zcdp.tex <==
\section{Extension to Other Privacy Definitions}

\subsection{R\'enyi Differential Privacy}

\begin{theorem}[Mironov, Proposition 3]
  Let ${\mathcal{M}}$ satisfy $(\alpha , \epsilon )$-RDP. Then ${\mathcal{M}}$ satisfies $(\epsilon ', \delta )$-differential privacy for all $\delta  > 0$ and $\epsilon ' = \epsilon  + \frac{\log (1/\delta )}{\alpha -1}$.
\end{theorem}

\begin{figure}
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  (\alpha ,\epsilon _{1})\otimes (\alpha ,\epsilon _{2}) \triangleq  (\alpha ,\epsilon _{1}+\epsilon _{2})
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \times  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  (\alpha ,\epsilon _{1})\oplus (\alpha ,\epsilon _{2}) \triangleq  (\alpha ,\epsilon _{1}+\epsilon _{2})
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}^{\dagger } \in  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \endgroup}\endgroup \end{tabularx}
\cr  (\alpha ,\epsilon )^{\dagger } \triangleq  (\alpha ,0)
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Gauss}}}
  ]{ \Gamma _{1} \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{n}}}\endgroup }]
  \\ \Gamma _{2} \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\alpha ]
  \\ \Gamma _{3} \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\epsilon ]
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{n{\otimes }\Gamma _{4}^{\dagger } \vdash  e_{4} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} }}}\endgroup }
     }{
     \Gamma _{1} \oplus  \Gamma _{2} \oplus  \Gamma _{3} \oplus  (\alpha ,\epsilon ){\otimes }\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma _{4}^{\dagger } }}}\endgroup }\rfloor  \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\alpha }}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\epsilon }}}}{=}e_{1},e_{2},e_{3}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ e_{4} }}}\endgroup }] \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}
  }
\end{mathpar}\endgroup 
\endgroup 
\caption{Type System Changes for R\'enyi Differential Privacy}
\end{figure}


\begin{figure}
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\otimes }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  \rho _{1}\otimes \rho _{2} \triangleq  \rho _{1}+\rho _{2}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}{\oplus }\underline{\hspace{0.66em}\vspace*{5ex}} \in  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{cost}}}} \endgroup}\endgroup \end{tabularx}
\cr  \rho _{1}\oplus \rho _2 \triangleq  \rho _{1}+\rho _{2}
\cr \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \underline{\hspace{0.66em}\vspace*{5ex}}^{\dagger } \in  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \rightarrow  {{\color{\colorMATH}\ensuremath{\operatorname{sens}}}} \endgroup}\endgroup \end{tabularx}
\cr  \rho ^{\dagger }  \triangleq  0
\vspace*{-1em}\end{gather*}\endgroup 
\endgroup 

\subsection{Zero-Concentrated Differential Privacy}

\begin{theorem}[Bun and Steinke, Lemma 3.5]
  Let ${\mathcal{M}}$ satisfy $\rho $-zCDP. Then ${\mathcal{M}}$ satisfies $(\epsilon , \delta )$-differential privacy for all $\delta  > 0$ and $\epsilon  = \rho  + \sqrt {4\rho \log (1/\delta )}$.
\end{theorem}

\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Gauss}}}
  ]{ \Gamma _{1} \vdash  e_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{n}}}\endgroup }]
  \\ \Gamma _{2} \vdash  e_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}[\rho ]
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{n{\otimes }\Gamma _{3}^{\dagger } \vdash  e_{3} \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}} }}}\endgroup }
     }{
     \Gamma _{1} \oplus  \Gamma _{2} \oplus  \rho {\otimes }\lfloor {\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ \Gamma _{3}^{\dagger } }}}\endgroup }\rfloor  \vdash  {{\color{\colorSYNTAX}\texttt{gauss}}}[{{\color{\colorSYNTAX}\texttt{r}}},{{\color{\colorSYNTAX}\ensuremath{\operatorname{\rho }}}}{=}e_{1},e_{2}][{\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}{{\color{\colorMATH}\ensuremath{ e_{3} }}}\endgroup }] \mathrel{:} {{\color{\colorSYNTAX}\texttt{real}}}
  }
\end{mathpar}\endgroup 
\endgroup 
\caption{Type System Changes for (Single-Parameter) Zero-Concentrated Differential Privacy}
\end{figure}

\FloatBarrier





==> type_level_reals.tex <==
\section{Type-level Real Variables}

\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{array}{rcrcl
  } \kappa  &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{kind}}}}  &{}\mathrel{\Coloneqq }{}& {{\color{\colorSYNTAX}\texttt{NAT}}} \mathrel{|} {{\color{\colorSYNTAX}\texttt{REAL}}}
  \cr  \rho  &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{tvar}}}}  &{} {}&
  \cr  R &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{texp}}}}  &{}\mathrel{\Coloneqq }{}& \rho  \mathrel{|} {.}\hspace{-1pt}{.}\hspace{-1pt}{.} 
  \cr  \Delta  &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{kcxt}}}}  &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{tvar}}}} \rightharpoonup  {{\color{\colorMATH}\ensuremath{\operatorname{kind}}}}
  \cr    &{} {}&         &{}\mathrel{\Coloneqq }{}& \{ \rho  \mathrel{:} \kappa ,{.}\hspace{-1pt}{.}\hspace{-1pt}{.}\} 
  \cr  T &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{subst}}}} &{}\triangleq {}& {{\color{\colorMATH}\ensuremath{\operatorname{tvar}}}} \rightharpoonup  {{\color{\colorMATH}\ensuremath{\operatorname{type}}}}
  \cr    &{} {}&         &{}\mathrel{\Coloneqq }{}& \{ \rho  \mapsto  \tau ,{.}\hspace{-1pt}{.}\hspace{-1pt}{.}\} 
  \cr  \tau  &{}\in {}& {{\color{\colorMATH}\ensuremath{\operatorname{type}}}}  &{}\mathrel{\Coloneqq }{}& {.}\hspace{-1pt}{.}\hspace{-1pt}{.} \mathrel{|} \forall \Delta ^{\prime}.\hspace*{0.33em}\tau  \multimap _{s} \tau  \mathrel{|} \forall \Delta ^{\prime}.\hspace*{0.33em} \tau @p,{.}\hspace{-1pt}{.}\hspace{-1pt}{.},\tau @p \multimap ^{*} \tau 
  \end{array}
\vspace*{-1em}\end{gather*}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Delta  \vdash  R \mathrel{:} \kappa  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Var}}}
  ]{ \rho \mathrel{:}\kappa  \in  \Delta 
     }{
     \Delta  \vdash  \rho  \mathrel{:} \kappa 
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Nat}}}
  ]{ }{
     \Delta  \vdash  n \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Real}}}
  ]{ }{
     \Delta  \vdash  r \mathrel{:} {{\color{\colorSYNTAX}\texttt{REAL}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Inf}}}
  ]{ }{
     \Delta  \vdash  \infty  \mathrel{:} {{\color{\colorSYNTAX}\texttt{REAL}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Plus}}}
  ]{ \Delta  \vdash  R_{1} \mathrel{:} \kappa 
  \\ \Delta  \vdash  R_{2} \mathrel{:} \kappa 
     }{
     \Delta  \vdash  R_{1} + R_{2} \mathrel{:} \kappa 
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Mult}}}
  ]{ \Delta  \vdash  R_{1} \mathrel{:} \kappa 
  \\ \Delta  \vdash  R_{2} \mathrel{:} \kappa 
     }{
     \Delta  \vdash  R_{1} \mathrel{\mathord{\cdotp }} R_{2} \mathrel{:} \kappa 
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Div}}}
  ]{ \Delta  \vdash  R_{1} \mathrel{:} \kappa 
  \\ \Delta  \vdash  R_{2} \mathrel{:} \kappa 
     }{
     \Delta  \vdash  R_{1} \mathrel{\mathord{\cdotp }} R_{2} \mathrel{:} \kappa 
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Root}}}
  ]{ \Delta  \vdash  R \mathrel{:} \kappa 
     }{
     \Delta  \vdash  \sqrt R \mathrel{:} {{\color{\colorSYNTAX}\texttt{REAL}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Log}}}
  ]{ \Delta  \vdash  R \mathrel{:} \kappa 
     }{
     \Delta  \vdash  \ln R \mathrel{:} {{\color{\colorSYNTAX}\texttt{REAL}}}
  }
\end{mathpar}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Delta  \vdash  \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Nat}}}
  ]{ }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{nat}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Static Nat}}}
  ]{ \Delta  \vdash  R \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
     }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{nat}}}[R]
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Real}}}
  ]{ }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{real}}}
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Static Real}}}
  ]{ \Delta  \vdash  R \mathrel{:} {{\color{\colorSYNTAX}\texttt{REAL}}}
     }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{real}}}[R]
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Matrix}}}
  ]{ \Delta  \vdash  R_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
  \\ \Delta  \vdash  R_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
  \\ \Delta  \vdash  \tau 
     }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{matrix}}}_{U}[R_{1},R_{2}](\tau )
  }
\and\inferrule*[lab={{\color{\colorTEXT}\textsc{\scriptsize Norm-Matrix}}}
  ]{ \Delta  \vdash  R_{1} \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
  \\ \Delta  \vdash  R_{2} \mathrel{:} {{\color{\colorSYNTAX}\texttt{NAT}}}
  \\ \Delta  \vdash  \tau 
  \\ \ell  \neq  U
     }{
     \Delta  \vdash  {{\color{\colorSYNTAX}\texttt{matrix}}}_{\ell }[R_{1},R_{2}]({{\color{\colorSYNTAX}\texttt{real}}})
  }
\and\inferrule*[lab={{\color{\colorMATH}\ensuremath{+}}}{{\color{\colorTEXT}\textsc{\scriptsize -F}}}
  ]{ \Delta  \vdash  \tau _{1}
  \\ \Delta  \vdash  \tau _{2}
     }{
     \Delta  \vdash  \tau _{1} + \tau _{2}
  }
\and\inferrule*[lab={{\color{\colorMATH}\ensuremath{\times }}}{{\color{\colorTEXT}\textsc{\scriptsize -F}}}
  ]{ \Delta  \vdash  \tau _{1}
  \\ \Delta  \vdash  \tau _{2}
     }{
     \Delta  \vdash  \tau _{1} \times  \tau _{2}
  }
\and\inferrule*[lab={{\color{\colorMATH}\ensuremath{\mathrel{\&}}}}{{\color{\colorTEXT}\textsc{\scriptsize -F}}}
  ]{ \Delta  \vdash  \tau _{1}
  \\ \Delta  \vdash  \tau _{2}
     }{
     \Delta  \vdash  \tau _{1} \mathrel{\&} \tau _{2}
  }
\and\inferrule*[lab={{\color{\colorMATH}\ensuremath{\multimap }}}{{\color{\colorTEXT}\textsc{\scriptsize -F}}}
  ]{ \Delta \uplus \Delta ^{\prime} \vdash  \tau _{1}
  \\ \Delta \uplus \Delta ^{\prime} \vdash  \tau _{2}
     }{
     \Delta  \vdash  \forall \Delta ^{\prime}.\hspace*{0.33em} \tau _{1} \multimap _{s} \tau _{2}
  }
\end{mathpar}\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Delta ,\Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHS}\renewcommand\colorSYNTAX{\colorSYNTAXS}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Delta ,\Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[flushleft,lab={{\color{\colorMATH}\ensuremath{\multimap }}}{{\color{\colorTEXT}\textsc{\scriptsize -I}}}
  ]{ \Delta \uplus \Delta ^{\prime} \vdash  \tau _{1}
  \\ \Delta \uplus \Delta ^{\prime},\Gamma \uplus \{ x\mathrel{:}_{s}\tau _{1}\}  \vdash  e \mathrel{:} \tau _{2}
     }{
     \Delta ,\Gamma  \vdash  \lambda x.e \mathrel{:} \forall \Delta ^{\prime}.\hspace*{0.33em} \tau _{1} \multimap _{s} \tau _{2}
  }
\and\inferrule*[flushleft,lab={{\color{\colorMATH}\ensuremath{\multimap }}}{{\color{\colorTEXT}\textsc{\scriptsize -E}}}
  ]{ \Delta ,\Gamma _{1} \vdash  e_{1} \mathrel{:} \forall \Delta ^{\prime}.\hspace*{0.33em} \tau _{1} \multimap _{s} \tau _{2}
  \\ \Delta ,\Gamma _{2} \vdash  e_{2} \mathrel{:} \tau _{1}[T/\Delta ^{\prime}]
     }{
     \Delta ,\Gamma _{1} \oplus  s{\otimes }\Gamma _{2} \vdash  e_{1}(e_{2}) \mathrel{:} \tau _{2}[T/\Delta ^{\prime}]
  }
\end{mathpar}\endgroup 
\endgroup 
\begingroup\renewcommand\colorMATH{\colorMATHP}\renewcommand\colorSYNTAX{\colorSYNTAXP}
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \Delta ,\Gamma  \vdash  e \mathrel{:} \tau  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[flushleft,lab={{\color{\colorMATH}\ensuremath{\multimap }}}{{\color{\colorTEXT}\textsc{\scriptsize -I}}}
  ]{ \Delta \uplus \Delta ^{\prime} \vdash  \tau _{1}
  \\ \Delta \uplus \Delta ^{\prime},\Gamma \uplus \{ x\mathrel{:}_{s}\tau _{1}\}  \vdash  e \mathrel{:} \tau _{1}
     }{
     \Delta ,\Gamma  \vdash  \lambda x.e \mathrel{:} \forall \Delta ^{\prime}.\hspace*{0.33em}\tau _{1} \multimap _{s} \tau _{2}
  }
\and\inferrule*[flushleft,lab={{\color{\colorMATH}\ensuremath{\multimap }}}{{\color{\colorTEXT}\textsc{\scriptsize -E}}}
  ]{ \Delta ,\Gamma  \vdash  e \mathrel{:} \forall \Delta ^{\prime}.\hspace*{0.33em}\tau _{1} \multimap _{s} \tau _{2}
     }{
     \Delta ,\{ x\mathrel{:}_{s}\tau _{1}[T/\Delta ^{\prime}]\} \oplus \Gamma  \vdash  e(x) \mathrel{:} \tau _{2}[T/\Delta ^{\prime}]
  }
\end{mathpar}\endgroup 
\endgroup 
\vspace*{-0.25em}\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \llbracket \underline{\hspace{0.66em}\vspace*{5ex}}\rrbracket  \in  {{\color{\colorMATH}\ensuremath{\operatorname{texp}}}} \times  ({{\color{\colorMATH}\ensuremath{\operatorname{tvar}}}} \rightharpoonup  {\mathbb{R}}\uplus \{ \infty \} ) \rightharpoonup  {\mathbb{R}}\uplus \{ \infty \}  \endgroup}\endgroup \end{tabularx}\vspace*{-1em}\end{gather*}\endgroup 
\begingroup\color{\colorMATH}\begin{mathpar}\begin{array}{rcl
  } \llbracket \rho \rrbracket (\nu )         &{}\triangleq {}& \nu (\rho )
  \cr  \llbracket n\rrbracket (\nu )         &{}\triangleq {}& n
  \cr  \llbracket r\rrbracket (\nu )         &{}\triangleq {}& r
  \end{array}
\and\begin{array}{rcl
  } \llbracket \infty \rrbracket (\nu )         &{}\triangleq {}& \infty 
  \cr  \llbracket R_{1}+R_{2}\rrbracket (\nu )     &{}\triangleq {}& \llbracket R_{1}\rrbracket (\nu ) + \llbracket R_{2}\rrbracket (\nu )
  \cr  \llbracket R_{1}\mathrel{\mathord{\cdotp }}R_{2}\rrbracket (\nu )     &{}\triangleq {}& \llbracket R_{1}\rrbracket (\nu ) \mathrel{\mathord{\cdotp }} \llbracket R_{2}\rrbracket (\nu )
  \end{array}
\and\begin{array}{rcl
  } \llbracket R_{1}/R_{2}\rrbracket (\nu )     &{}\triangleq {}& \llbracket R_{1}\rrbracket (\nu ) / \llbracket R_{2}\rrbracket (\nu )
  \cr  \llbracket \sqrt R\rrbracket (\nu )        &{}\triangleq {}& \sqrt {\llbracket R\rrbracket (\nu )}
  \cr  \llbracket \ln R\rrbracket (\nu )       &{}\triangleq {}& \ln \llbracket R(\nu )\rrbracket 
  \end{array}
\end{mathpar}\endgroup 

